Modeling Dynamic Hand-Object Interactions with Applications to Human-Robot Handovers

Humans frequently grasp, manipulate, and move objects. Interactive systems assist humans in these tasks, enabling applications in Embodied AI, human-robot interaction, and virtual reality. However, current methods in hand-object synthesis often neglect dynamics and focus on generating static grasps. The first part of this dissertation introduces dynamic grasp synthesis, where a hand grasps and moves an object to a target pose. We approach this task using physical simulation and reinforcement learning. We then extend this to bimanual manipulation and articulated objects, requiring fine-grained coordination between hands. In the second part of this dissertation, we study human-to-robot handovers. We integrate captured human motion into simulation and introduce a student-teacher framework that adapts to human behavior and transfers from sim to real. To overcome data scarcity, we generate synthetic interactions, increasing training diversity by 100x. Our user study finds no difference between policies trained on synthetic vs. real motions.

==> chapters/01_introduction/content/thesis_statement.tex <==
\section{Thesis Statement}


==> chapters/02_related_work/content/datasets.tex <==
\input{\dir/tables/datasets}

\subsection{Datasets}
There has been a surge of datasets introduced that capture hand-object interaction~\cite{brahmbhatt2019contactdb, hampali2020honnotate, moon2020interhand2.6m, taheri2020grab, zhang2016magnetic, garciahernando2018first, brahmbhatt2020contactpose, chao2021dexycb, kwon2021h2o, ye2021h2o, wang2023dexgraspnet, yang2022OakInk, zhan2024oakink2, jian2023affordpose, zhu2024contactart, liu2024taco}. We provide an overview of the most relevant datasets in \Tab{compare_datasets}. Synthetic datasets model single static hand-object grasps, which are obtained either via simulation in ObMan \cite{hasson2019learning} or manual annotation as in AffordPose \cite{jian2023affordpose}. 
ContactArt \cite{zhu2024contactart} collects interactions with articulated objects in physical simulation directly via teleoperation. Also focusing on articulated objects, ARCTIC \cite{fan2023arctic} is the only dataset that includes bi-manual manipulation, the full human body, and dexterous manipulation of objects. It comprises 11 diverse object shapes, such as an espresso machine, a ketchup bottle, and a laptop. HO3D \cite{hampali2020honnotate} and H2O-3D \cite{hampali2022keypoint} are datasets that capture hand and object with severe occlusion from each other. HO3D \cite{hampali2020honnotate} focuses on right-handed interactions with 10 objects, whereas H2O-3D \cite{hampali2022keypoint} comprises two-handed interactions. Similarly, FHPA \cite{garciahernando2018first} is a dataset that contains manipulation of objects from ego-centric view with a single hand, and H2O \cite{kwon2021h2o} extends this setting to bi-manual manipulations.
OakInk \cite{yang2022OakInk} comprises dexterous manipulation of 100 objects with one hand with a specific focus on taking into consideration the affordances of the objects. In OakInk2 \cite{zhan2024oakink2}, this setting is extended to bi-manual manipulation and multi-object affordances. DexYCB \cite{chao2021dexycb} includes 20 objects and 1000 left- and right-handed sequences of participants grasping YCB objects \cite{calli2015ycb} and lifting them above a table. Core4D \cite{zhang2024core4d} is a dataset that models collaborative tasks between multiple humans, such as carrying boxes or tables together. There are many more recent efforts that capture human-object interactions with such larger objects \cite{zhang2023neuraldome, zhang2024hoi, huang2024intercap, jiang2023iccv}, and we refer the reader to \cite{zhang2024core4d} for a more detailed overview. The GRAB dataset \cite{taheri2020grab} includes 51 objects, 10 participants, and captures the full-body of the human using the SMPL-X parametric body model \cite{pavlakos2019smplx}. It contains sequences of object manipulations with one or two hands, such as grasping an apple and passing it from one hand to another before taking a bite. It also includes semantic action labels that describe the manipulation type. TACO \cite{liu2024taco} captures the task of bi-manual multi-object manipulation, going beyond previous datasets that are mostly limited to single object interaction. An example of such a task is stirring food in a bowl with a spatula. The largest amount of diverse object shapes (800 objects) and sequences among the non-synthetic datasets is available in HOI4D \cite{liu2022hoi4d} that comprises single handed manipulation sequences.  
Overall, we observe that most available datasets are limited in terms of object diversity and the number of available motion sequences. Only the synthetic ObMan dataset \cite{hasson2019learning} includes more than one thousand objects. However, ObMan only contains single static grasps. Furthermore, most datasets focus on the simplified setting of single-handed grasping of non-articulated objects. In the first part of this thesis, we take a step towards modeling hand-object interactions synthetically. We start with a single-handed setting of rigid object grasping in D-Grasp (see Chapter \ref{ch:hoi_generation:dgrasp}) and extend it to bi-manual manipulation and articulated objects in ArtiGrasp (see Chapter \ref{ch:hoi_generation:artigrasp}).





==> chapters/04_hoi_generation/artigrasp/FIG/com_arti.tex <==

\begin{figure}
  \centering
  \begin{subfigure}{1.0\linewidth}
        \centering
        {\includegraphics[width=0.3\textwidth]{\dir/artigrasp/figures/seqs/arti_comparison/pd_arti_1.png} 
     \includegraphics[width=0.3\textwidth]{\dir/artigrasp/figures/seqs/arti_comparison/pd_arti_2.png}
     \includegraphics[width=0.3\textwidth]{\dir/artigrasp/figures/seqs/arti_comparison/pd_arti_3.png}}
    \caption{PD+IK}
  \end{subfigure}
  \hfill
  \begin{subfigure}{1.0\linewidth}
        \centering
        {\includegraphics[width=0.3\textwidth]{\dir/artigrasp/figures/seqs/arti_comparison/dgrasp_arti_1.png} 
     \includegraphics[width=0.3\textwidth]{\dir/artigrasp/figures/seqs/arti_comparison/dgrasp_arti_2.png}
     \includegraphics[width=0.3\textwidth]{\dir/artigrasp/figures/seqs/arti_comparison/dgrasp_arti_3.png}}
    \caption{D-Grasp}
  \end{subfigure}
  \hfill
  \begin{subfigure}{1.0\linewidth}
        \centering
        {\includegraphics[width=0.3\textwidth]{\dir/artigrasp/figures/seqs/arti_comparison/ours_arti_1.png} 
     \includegraphics[width=0.3\textwidth]{\dir/artigrasp/figures/seqs/arti_comparison/ours_arti_2.png}
     \includegraphics[width=0.3\textwidth]{\dir/artigrasp/figures/seqs/arti_comparison/ours_arti_3.png}}
    \caption{Ours}
  \end{subfigure}
  \caption{\textbf{Qualitative evaluation of articulation.} When evaluated only on articulation, both PD+IK and D-Grasp often fail at the task. On the other hand, our method can articulate the object successfully.}
    \label{fig:arti:comparison_arti}
\end{figure}

==> chapters/04_hoi_generation/artigrasp/FIG/com_grasp.tex <==
\begin{figure}
  \centering
  \begin{subfigure}{1.0\linewidth}
    \centering
    {\includegraphics[width=0.3\textwidth]{\dir/artigrasp/figures/seqs/grasp_comparison/pd_1.png}
     \includegraphics[width=0.3\textwidth]{\dir/artigrasp/figures/seqs/grasp_comparison/pd_2.png}
     \includegraphics[width=0.3\textwidth]{\dir/artigrasp/figures/seqs/grasp_comparison/pd_3.png}}
    \caption{PD+IK}
  \end{subfigure}
  \hfill
  \begin{subfigure}{1.0\linewidth}
        \centering
    {\includegraphics[width=0.3\textwidth]{\dir/artigrasp/figures/seqs/grasp_comparison/dgrasp_1.png} 
     \includegraphics[width=0.3\textwidth]{\dir/artigrasp/figures/seqs/grasp_comparison/dgrasp_2.png}
     \includegraphics[width=0.3\textwidth]{\dir/artigrasp/figures/seqs/grasp_comparison/dgrasp_3.png}}
    \caption{D-Grasp}
  \end{subfigure}
  \hfill
  \begin{subfigure}{1.0\linewidth}
        \centering
        {\includegraphics[width=0.3\textwidth]{\dir/artigrasp/figures/seqs/grasp_comparison/ours_1.png}
     \includegraphics[width=0.3\textwidth]{\dir/artigrasp/figures/seqs/grasp_comparison/ours_2.png}
     \includegraphics[width=0.3\textwidth]{\dir/artigrasp/figures/seqs/grasp_comparison/ours_3.png}}
    \caption{Ours}
  \end{subfigure}
  \caption{\textbf{Qualitative evaluation of grasping.} When evaluated only on grasping, PD+IK often fails to successfully grasp the object. On the other hand, D-Grasp and ours succeed at the task.}
    \label{fig:arti:comparison_grasp}
\end{figure}

==> chapters/04_hoi_generation/artigrasp/FIG/sequences.tex <==
\begin{figure}
	\centering
\includegraphics[width=0.47\textwidth]{\dir/artigrasp/figures/seqs/individual_seqs/individual.pdf}
\caption{\textbf{Qualitative outputs of our method.} We provide more sequences for grasping and articulation, which are generated by our method with a single pair of hand pose reference label per interaction. Each sequence is shown from left to right.}
\label{fig:arti:more_samples}
\end{figure}


==> chapters/04_hoi_generation/artigrasp/sections/0_abstract.tex <==
\begin{abstract}
\vspace{-2mm}
We present \methodname, a novel method to synthesize bi-manual hand-object interactions that include grasping and articulation. This task is challenging due to the diversity of the global wrist motions and the precise finger control that are necessary to articulate objects. \methodname\ leverages reinforcement learning and physics simulations to train a policy that controls the global and local hand pose. Our framework unifies grasping and articulation within a single policy guided by a single hand pose reference. Moreover, to facilitate the training of the precise finger control required for articulation, we present a learning curriculum with increasing difficulty. It starts with single-hand manipulation of stationary objects and continues with multi-agent training including both hands and non-stationary objects. To evaluate our method, we introduce \task, a task that involves bringing an object into a target articulated pose. This task requires grasping, relocation, and articulation. We show our method's efficacy towards this task. We further demonstrate that our method can generate motions with noisy hand-object pose estimates from an off-the-shelf image-based regressor.  Project page: \href{https://eth-ait.github.io/artigrasp/}{https://eth-ait.github.io/artigrasp/}.
\end{abstract}


==> chapters/04_hoi_generation/artigrasp/sections/2_related_work.tex <==
% Head 1
\section{Related Work}
\label{related}

\input{sections/tables/related_work}

We categorize related research into human grasp generation, motion synthesis, and dexterous robotic hand manipulation. \refTab{tab:related_work} compares different hand-object motion generation methods to ours. 

\subsection{Hand-object Reconstruction and Synthesis}

There has been a surge of large-scale datasets introduced for modeling hand-object interaction~\cite{brahmbhatt2019contactdb, hampali2020ho3d, brahmbhatt2020contactpose, chao2021dexycb, kwon2021h2o, wang2023dexgraspnet}. Recent datasets include interactions with articulated objects~\cite{fan2023arctic,zhu2023contactart,liu2022ho4d,xu2021d3d}. Methods that are being developed with these datasets can be split into two categories: 1) \textit{hand-object reconstruction}; 2) \textit{hand grasp synthesis}.

The goal of \textit{hand-object reconstruction}~\cite{hasson2019obman,liu2021semi,Yang_2021_CPF,grady2021contactopt,Hasson2020photometric,tekin2019ho,corona2020ganhand,zhou2020monocular, zhou2022toch, ziani2022tempclr} is to estimate the \threeD hand and object surfaces from RGB images. Methods mostly leverage deep learning models, for example, by using 3D supervision and synthetic images~\cite{hasson2019obman}, temporal models~\cite{tekin2019ho}, or by integrating adversarial priors and contact constraints~\cite{corona2020ganhand}. Others focus on the denoising of pose estimates~\cite{grady2021contactopt, zhou2022toch}.

In \textit{hand grasp synthesis}, the goal is to generate static hand grasps given an object mesh as input. 
%
Corona \etal~\cite{corona2020ganhand} first generate the grasp type and then refine the grasp pose accordingly. 
%
Karunratanakul \etal~\cite{karunratanakul2021halo} introduce a part-based implicit hand model for grasp synthesis.
%
Hidalgo-Carvajal \etal~\cite{hidalgo2022objectcentric} use 10 pre-defined poses to predict infeasible grasping areas and feasible hand poses.
%
Some methods use contact information to predict or refine the grasp configuration~\cite{jiang2021graspTTA, li2023contact2grasp, ye2012synthesis, yang2021ArtiBoost, grady2021contactopt}. 
Moreover, physics-based optimization can be leveraged to improve the initial grasping pose~\cite{wang2023dexgraspnet, wu2022learning}. 
Han \etal~\cite{han2023vrhand} optimize a single reference grasp pose for grasping different objects in virtual reality. 
Some other approaches focus on more general tasks, such as generating grasps for dexterous hands and grippers~\cite{li2023gendexgrasp} or using implicit representations~\cite{karunratanakul2020grasping} for grasping and reconstruction.

The methods above are orthogonal to ours.
They do not generate hand motion but provide useful static grasp poses that we can potentially leverage to synthesize motions involving grasping and manipulating objects.

\subsection {Motion Synthesis}
The synthesis of human motion is a long-standing problem in graphics and computer vision~\cite{ Aksan_2019_ICCV, aksan2020motiontransformer, ghosh2017learning,holden2015tog, holden2016tog}. 
Recently, there have been methods that synthesize human body motion interacting with static scenes~\cite{hassan2021samp, cao2020long, starke2020local,zhang2022couch,wang2021scene,lee2023locomotionactionmanipulation, huang2023diffusionbased, zhang2023roam}, such as sitting on a chair or sofa.
This line of work focuses on the human body motion and does not generate motions of hand-object interaction.
There are methods that generate \fullbody grasping motion~\cite{taheri2021goal, ghosh2022imos, li2023taskoriented, wu2022saga}, but they are purely data-driven approaches without physics. They either require a post-processing optimization for the object motion~\cite{ghosh2022imos}, or only generate the approaching motion until grasping~\cite{wu2022saga, taheri2021goal}. Recent work has also explored integrating physics simulations into pose reconstruction~\cite{yuan2021simpoe, shimada2020physcap, shimada2021neural}, synthesis~\cite{xie2021iccv}, and even coarse human-object interaction pipelines~\cite{chao2021learning,luo2022embodied,hassan2023synthesizing}. However, these physics-based methods focus on the body motion and do not model hands to capture fine-grained hand-object interactions. In contrast, we omit the human body and focus specifically on bi-manual hand-object manipulation.

Similar to ours, some recent methods also focus on dexterous hands~\cite{wang2019learning} and generate interactive sequences that include physics~\cite{christen2022dgrasp, braun2023physically}, articulated objects~\cite{zheng2023cams}, or bi-manual manipulation~\cite{zhang2021manipnet}. Wang \etal~\cite{wang2019learning} generate multi-step human-object interactions from videos without physics. Christen \etal~\cite{christen2022dgrasp} generate natural grasping sequences from static grasp references in a physics simulation, but focus on rigid objects and only consider one hand. Zheng \etal~\cite{zheng2023cams} presents a data-driven method to synthesize single-hand pose sequences for articulated objects and uses post-optimization to make the sequences more physically plausible. 
Zhang \etal~\cite{zhang2021manipnet} predict finger poses for two-hand object interaction. However, they require the full trajectory of the wrist and object at inference time. 
In our work, we generate object and wrist motions through interaction with the objects in a physics simulation.
 
\subsection{Dexterous Robotic Hand Manipulation}
Dexterous robotic manipulation is often addressed by leveraging physics simulation and reinforcement learning with robotic hands~\cite{she2022grasping, ye2023grasping, liu2023dexrepnet, rajeswaran2018learning, garciahernando2020iros}. Some common strategies to learn to grasp different objects include data augmentation~\cite{Chen2022LearningRR}, curriculum learning~\cite{zhang2023learning}, or improving the movement re-targeting from human demonstrations to the robot hand in a physics simulation~\cite{qin2022dexmv, chen2022dextransfer, liu2023dexrepnet}. Other approaches include tele-operated sequences as training data~\cite{rajeswaran2018learning} or use demonstrations as prior and predict residual actions~\cite{garciahernando2020iros}. Alternatively, a parameterized reward function based on demonstrations can be used~\cite{christen2019hri}. All of these methods rely on demonstration of entire grasping sequence. In contrast, our method only requires static hand pose references, which are easier to obtain. 

To alleviate the need for expert demonstrations, some methods are formulated as pure RL problems~\cite{openai2018dexterous, chen2021simple}. Chen \etal~\cite{chen2022humanlevel} propose a benchmark for two-hand manipulation tasks and use standard RL algorithms. However, the hand poses remain rather unnatural. They mitigate this by fine-tuning with a human preference reward~\cite{ding2023learning}. 
Mandikal and Grauman~\cite{mandikal2020graff} train an affordance-aware policy for grasping. They further introduce a hand pose prior learned from YouTube videos to achieve more natural hand configurations~\cite{mandikal2021dexvip}. However, they only consider a single pose per object. Qin \etal~\cite{qin2023dexpoint} achieve grasping objects or opening doors with noisy point clouds from a single camera. Xu \etal~\cite{xu2023unidexgrasp} and Wan \etal~\cite{wan2023unidexgrasp} generate grasp sequences on objects with point clouds. Yang \etal~\cite{yang2022chop} focus on planning interactions with chopsticks that are already in the hand from the start. All these methods consider a single robotic hand and focus mostly on rigid objects, while our method can handle two hands for both grasping and articulation of different objects with a single policy. Chen \etal~\cite{NEURIPS2022BidexHand} propose a benchmark for bi-manual manipulation with different rewards and separately trained policies for each individual task and object. In contrast, our method learns a general policy across different articulated objects for approaching, grasping and articulating.





==> chapters/04_hoi_generation/artigrasp/tables/main_result.tex <==
\begin{table}[t]
\centering

\begin{minipage}{\columnwidth}
\begin{center}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l|ccc|ccc}
   \toprule
    & \multicolumn{3}{c|}{Grasping} & \multicolumn{3}{c}{Articulation} \\
    \midrule
    Model & Suc. G $\uparrow$ & PE $\downarrow$ & AE $\downarrow$ & Suc. A $\uparrow$ & AAE $\downarrow$ & SD $\downarrow$ \\
    \midrule
    PD+IK                                             & 0.13 & 1.20 & 1.50 & 0.28 & 0.80 & 0.39 \\
             \dgrasp & \textbf{0.72} & \textbf{0.12} & \textbf{0.62} & 0.22 & 0.93 & 0.49 \\
             Ours & 0.71 & 0.13 & 0.69 & \textbf{0.55} & \textbf{0.57} & \textbf{0.01} \\
             % \midrule
              % Improve over D-Grasp & -0.01 & -0.01 & -0.07 & 0.33 & 0.36 & 0.48 \\
   \bottomrule
\end{tabular}
} %%% resize box
\end{center}

\end{minipage}
\caption{\heading{Quantitative comparison for grasping and articulation tasks} When the tasks are decoupled, we find that our method outperforms the baselines on articulation and performs comparably to D-Grasp on grasping.}
\label{tab:one}

\end{table}


==> chapters/04_hoi_generation/artigrasp/tables/recon_result.tex <==
\begin{table}%


\begin{minipage}{\columnwidth}
\begin{center}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l|ccc|ccc}
   \toprule
   & \multicolumn{3}{c|}{Grasping} & \multicolumn{3}{c}{Articulation} \\
    \midrule
    Models & Suc.G $\uparrow$ & PE $\downarrow$ & AE $\downarrow$ & Suc.A $\uparrow$ & AAE $\downarrow$ & SD $\downarrow$\\
   \midrule
    % PD+IK     & 0 & 0 & 0 & 0 & 0 & 0  \\
    \dgrasp   & 0.60 & \textbf{0.16} & \textbf{0.78} & 0.20 & 1.07 & 0.63  \\
    Ours    & \textbf{0.64} & \textbf{0.16} & 0.80 & \textbf{0.54} & \textbf{0.55} & \textbf{0.01}   \\
    \midrule
    Ours$^{*}$        & 0.67 & 0.14 & 0.95 & 0.54 & 0.53 & 0.01  \\ 
   \bottomrule
\end{tabular}
}  % resizebox

\end{center}


\end{minipage}
\caption{Results with reconstructed hand pose references When evaluated with predictions from images, we observe a minor drop in performance for grasping and articulation compared to mocap data. However, the overall performance shows that our method can handle noisy estimates. The asterisk (*) denotes using hand pose references from mocap. }
\label{tab:arti:recon}

\end{table}%


==> chapters/04_hoi_generation/content/conclusion.tex <==
\chapter{Summary \& Insights}
\label{ch:hoi:conclusion}

\paragraph{Summary}
We introduced two works in this part, D-Grasp and ArtiGrasp, that synthesize hand-object interactions in 4D. In D-Grasp, we proposed the first method that generates dynamic hand-object sequences from sparse grasp references for a single hand and with rigid objects. In ArtiGrasp, we extended the setting to include bi-manual manipulation and articulated objects. By leveraging physical simulation, we ensured that the generated outputs are physically plausible. To address the sparsity in available hand-object data, we utilized reinforcement learning and proposed a general reward function. As both of these models are conditioned on grasp references, we showed that it is possible to generate such references via off-the-shelf image-based pose estimation or grasp synthesis. In our experiments, we demonstrated that our frameworks can generate realistic and natural sequences of object interaction, and that even long sequences with multi-object interaction can be synthesized. 

\paragraph{Implications}
We presented the first methods that generate sequential human-like hand-object interaction motions from sparse reference inputs. These methods open up a new perspective of modeling human-object interaction and have implications for different downstream applications. The generation of synthetic data at scale can potentially be useful in hand-pose estimation tasks, especially when the 3D data is combined with photo-realistic rendering techniques. Moreover, it could serve as demonstration data for teaching dexterous grasping in robotics. Another interesting direction is the use of synthetic human motion data is in Embodied AI, where it could be used to simulate human counterparts for teaching human-robot interactions. We will explore use of such data in human-robot interaction in Part \ref{part:h2r}.

\paragraph{Limitations and Future Work}
% 
In both D-Grasp and ArtiGrasp, the frameworks require access to a single hand grasp reference. We showed how such references can be obtained in practice on a small scale, e.g., by using image-based pose estimation, yet there are limiting assumptions that hinder the generation of hand-object interaction at large scale. First, we assume access to an object mesh, which in the real world is often not available, especially when extracting grasp references from images. In the future, this can potentially be alleviated by utilizing methods that reconstruct the object mesh along with the hand pose estimation \cite{fan2024hold}. As we have also demonstrated in our experiments, grasp references can be obtained from grasp synthesis \cite{jiang2021hand}. However, these methods themselves are limited in their generalization ability to a large scale and variety of objects, mostly due to the small amount of available high-quality training data. On the other hand, optimization-based methods can overcome such limitations, but at the cost of increased time complexity \cite{miller2004graspit, turpin2022grasp}. Moreover, both learning-based and optimization-based synthesis methods are yet to display capabilities of generating functional grasps. For instance, a bottle should be grasped by its top to be opened or a hammer should be picked up by its handle. To achieve such grasping behavior, models need to gain an understanding of object geometry as well as functionality, and be able to link this to grasp generation. Being able to generate such grasp references would enable our model to learn meaningful grasping behavior on novel objects.

% Disembodied Hand
In our works, we decouple the hand from the rest of the body and focus on grasping with such a disembodied hand. However, in more realistic environments, modeling the entire human body is important for certain downstream applications such as embodied AI or pedestrian modeling in autonomous driving. Furthermore employ rigid body physical simulation, treating both the hand and object as rigid bodies. However, the human hand and many objects humans interact with are deformable. Therefore, our approach has limitations in accurately modeling such interactions. Exploring simulations that account for hand deformation and learning to manipulate deformable objects presents exciting opportunities for future research.

% Grasp and Relocation
In the presented works, we focused on the grasping of objects and its subsequent relocation to some target pose. In reality, however, most interactions with objects go beyond simple grasping and moving the objects. More often, humans manipulate the objects and interact with them in functional ways. How to model manipulation of objects is an on-going area of research. In ArtiGrasp, we took a step towards human-like manipulation of articulated objects. A closer look at the generated sequences shows that the interaction is primarily stable grasping combined with wrist movements to articulate the objects, e.g., grasp the top of the box and then open it by moving the wrist in an upward motion. Our models have yet to exhibit more fine-grained manipulations where the finger poses change during interaction. Most often, existing methods either use a fixed hand to learn fine-grained object manipulations \cite{openai2018learning, chen2021simple} or focus on grasping as in our works. Models that combine the best of both worlds would enable more human-like interactions. 

% Long horizon tasks
Interactions would ideally also include longer horizon and multi-object manipulation. While we demonstrated in ArtiGrasp (see \figref{fig:arti:long_sequence}) that such long sequences can be composed, there are a lot of hand-designed components to make this work. In particular, the movement of the hands between different objects is done using heuristics, the order of actions is pre-defined, and each hand pose reference is hand-picked to enable smooth transitions. Future work could investigate how to generate long sequences automatically or leverage more user-friendly inputs, such as language.  

Since we are operating purely in physical simulation, we made assumptions about access to privileged information. Hence, applying our framework to robotic dexterous grasping in the real world is challenging, as this information may not be directly available. For instance, we use properties such as the object's pose, velocity, physical properties, and geometry. Furthermore, we utilize force sensors on the hand to indicate contacts. In real world settings, these properties are not directly available and have to either be measured beforehand or estimated. Moreover, predicting these properties will introduce noise into the measurements, and the method has to be robust against imperfect sensing. Such robustness is especially important in real world dexterous grasping, because small perturbations in object pose may already lead to unsuccessful grasps. In addition to the input modalities, one potential way to overcome this is by distilling a privileged teacher policy into a student policy that does only have access to information that is directly available in the real world, e.g., a policy with access to vision-based inputs and proprioceptive information \cite{wan2023unidexgrasp++, chen2021simple}. Another possibility is to use real-world data for the training of certain components of the framework \cite{hwangbo2019learning}. 

\paragraph{Follow-up work}
In the meantime, we have been able to address some of the aforementioned limitations in follow-up works that are outside the scope of this thesis. We will now briefly discuss how we tackled some of these limitations.

To address the limitation of object generalization of our frameworks, we propose GraspXL (\figref{fig:hoi:graspxl}), a novel method that is trained on 58 diverse object shapes and can generate grasping motions for over 500k objects \cite{zhang:2024:graspxl}. Unlike D-Grasp and ArtiGrasp, it does not rely on grasp references. Our model is trained using a general reward function and conditioned on a combination of objectives, such as approaching direction, affordance area to grasp, and the wrist rotation relative to the object. It uses an approximation of signed-distance function to learn about local geometry of objects. By training over a large variety of objectives and 58 distinct object geometries, GraspXL is able to generalize to an unprecedented scale of unseen object geometry. It can also be trained across different hand morphologies, such as different anthropomorphic robotic hands, which we show in our experiments.

To address the limitation of a floating, disembodied hand that is not subjected to bio-mechanical constraints, we propose a novel framework that learns to grasp and move objects with a full-body avatar \cite{braun:2023:physically} (\figref{fig:hoi:fbg}). Although we again make use of physical simulation and reinforcement learning, training a full-body character in physical simulation solely through a hand-crafted reward function will not lead to natural behavior. Therefore, we learn decoupled priors for the body and the hand in physical simulation that learn to imitate motions from existing full-body hand-object dataset \cite{taheri2020grab} through adversarial training \cite{peng2022ase}. This provides us with two latent spaces that can generate natural hand and body motions. Leveraging these priors, we train a downstream policy that directly samples in these latent spaces to learn object interactions. We propose a reward function similar to D-Grasp, but with additional incentives to follow root and wrist trajectories. This yields a policy that can be conditioned on arbitrary wrist trajectories, such as grasping an object from a table and moving it in a circular or zig-zag motion. This framework, however, still depends on coupled human-object trajectories for training the priors and a hand-pose reference at inference time for guidance, which limits the generalization ability to novel objects and trajectories. To address these simplifying assumptions, we propose Omnigrasp \cite{luo:2024:grasping}, a framework that learns to grasp over 1200 diverse object shapes with a full-body avatar. Our key insight is that learning a strong human motion prior is key for generalizable grasping in physical simulation. We achieve this by leveraging a large scale human motion dataset, AMASS \cite{mahmood2019amass}, with randomized actions for the hands to train our prior model. In downstream training, we sample from the prior and use a simple yet effective reward to track object trajectories. Therefore, we successfully eliminated the requirement of coupled human-object motion data and a grasp reference at inference. 

\begin{figure}[t!]
    \centering
    % Left figure
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth, trim={0 0 800 0}, clip]{\dir/content/figures/graspxl.jpg}
        \caption{GraspXL \cite{zhang:2024:graspxl}}
        \label{fig:hoi:graspxl}
    \end{subfigure}
    \hfill
    % Trimmed left half of the third figure
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth, trim={0 0 867 0}, clip]{\dir/content/figures/fullbody_grasp.png}
        \caption{Full-Body Grasping \cite{braun:2023:physically}}
        \label{fig:hoi:fbg}
    \end{subfigure}
        \hfill
     \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \begin{overpic}
        [width=\textwidth, trim={0 0 0 155}, clip]{\dir/content/figures/diffh2o.png}
        \put(10,95){\small{ "Drink from} }
        \put(10,85){ \small {the wineglass"}}
        \end{overpic}
        \caption{DiffH2O \cite{christen:2024:diffh2o}}
        \label{fig:hoi:diffh2o}
    \end{subfigure}
    \caption{In our follow-up works, we address several limitations: (a) In GraspXL \cite{zhang:2024:graspxl}, we generalize hand-object interactions to over 500k+ objects and different hand morphologies. (b) In \cite{braun:2023:physically}, we model the full human body and synthesize grasping motions that can follow arbitrary object target trajectories. (c) In DiffH2O \cite{christen:2024:diffh2o}, we generate hand-object interactions based on text descriptions, such as "drink from the wineglass".}
\end{figure}


Lastly, we go beyond our previous works that focus mostly on grasping and subsequent relocation or articulation of objects in our work DiffH2O \cite{christen:2024:diffh2o}. In this project, we build on the recent success of motion diffusion models in learning to generate human motions based on text descriptions (\figref{fig:hoi:diffh2o}). We present the first framework that allows synthesizing hand-object sequences based on language descriptions for unseen objects. Our technical contributions in this work are three-fold. First, we propose a two-stage process that decoupled grasping from text-based manipulation of objects. We leverage diffusion models for both stages. Next, we propose a compact representation that includes predictions in PCA-space to achieve natural predictions of hand poses despite the lack of large scale hand-object datasets. Lastly, we introduce a technique dubbed grasp guidance that can be used at inference time to incentivize the diffusion model to pass through single frame grasp references. We show in our experiments that such a guidance signal helps in achieving more physically plausible interactions. To foster research in text-based hand-object interaction synthesis, we further contribute detailed textual descriptions of the GRAB \cite{taheri2020grab} dataset. In our experiments, we compare against previous models for human motion diffusion models \cite{tevet2023human, karunratanakul2023guided} and action-based synthesis of HOI \cite{ghosh2023imos}. We show both qualitatively and quantitatively that our method is able to generate more natural and plausible hand-object interactions.

==> chapters/04_hoi_generation/content/introduction.tex <==
\chapter{Introduction}
\label{ch:hoi:introduction}



==> chapters/04_hoi_generation/dgrasp/sections/00_abstract.tex <==
\begin{abstract}
\vspace{-1em}
We introduce the \taskname~task: given an object with a known 6D pose and a grasp reference, our goal is to generate motions that move the object to a target 6D pose. 

This is challenging, because it requires reasoning about the complex articulation of the human hand and the intricate physical interaction with the object. 
%
We propose a novel method that frames this problem in the reinforcement learning framework and leverages a physics simulation, both to learn and to evaluate such dynamic interactions. 
%
A hierarchical approach decomposes the task into low-level grasping and high-level motion synthesis. 
It can be used to generate novel hand sequences that approach, grasp, and move an object to a desired location, while retaining human-likeness. 
%
We show that our approach leads to stable grasps and generates a wide range of motions. 
%
Furthermore, even imperfect labels can be corrected by our method to generate dynamic interaction sequences. Video and code are available at: \footnotesize{\url{https://eth-ait.github.io/d-grasp/}}.
\vspace{-0.8cm}
\end{abstract}

==> chapters/04_hoi_generation/dgrasp/sections/02_related_work.tex <==
\section{Related Work}

\begin{figure*}[t]
\begin{center}
   \includegraphics[width=0.98\textwidth]{images/model_overview_v4_cam_ready.pdf}
\end{center}
\vspace{-0.4cm}
   \caption{\textbf{Method Overview:} Taking a single, static grasp label  $\grasplabel$ and a target object 6D pose $\mathbf{T}_g$ as input (leftmost), \methodname produces sequences of dynamic hand-object interactions (rightmost). To do so, we propose a hierarchical framework that consists of a low-level grasping policy $\boldsymbol{\pi}_g(\cdot)$ and a high-level motion synthesis module. In the \emph{grasping} phase, only the grasping policy is active and finds a stable grasp on the object. In the subsequent \emph{motion synthesis} phase, both the grasping policy and the motion synthesis module act concurrently. The actions $\mathbf{a}$ consist of joint targets. These are combined and passed to a PD-controller that computes the required torques $\boldsymbol{\tau}$ to control a MANO-based hand model in a physics simulation. The physics simulation updates the state $\mathbf{s}$ which serves as input to a reward formulation (\secref{sec:dgrasp:method_reward}) that forms our supervision signal and incentivizes the hand to approach and grasp the object and to move it to the target 6D pose. We introduce two feature extraction layers ($\phi(\cdot)$ an $\psi(\cdot)$) that utilize the environment state $\mathbf{s}$ and grasp label $\grasplabel$ to find a suitable representation for the grasping policy and the motion synthesis module.}
\vspace{-0.2cm}
\label{fig:dgrasp:method_overview}
\end{figure*}

\textbf{Human Grasp Prediction}
Recently, hand-object interaction has received much research attention. This growth is accelerated by the introduction of datasets that contain both hand and object annotations \cite{brahmbhatt2019contactdb, brahmbhatt2020contactpose, corona2020ganhand, taheri2020grabnet, hampali2020ho3d, chao2021dexycb, kwon2021h2o}. 
Leveraging this data, a large number of methods attempt to estimate grasp parameters, such as the hand and object pose, directly from RGB images \cite{karunratanakul2020grasping, yang2021cpf, doosti2020hope, tekin2019h+, hasson2019learning, hasson2020leveraging, liu2021semi, cao2021reconstructing}. Some predict the mesh of the hand and the object directly \cite{hasson2019learning}, or assume a known object and predict its 6DoF in addition to the hand \cite{hasson2020leveraging, cao2021reconstructing, yang2021cpf, liu2021semi}. Others predict 3D keypoints and 6 DoF pose of the object \cite{doosti2020hope, tekin2019h+} or produce an implicit surface representation of the grasping hands \cite{karunratanakul2020grasping}. To improve the prediction accuracy of the grasp, many of these works incorporate additional contact losses \cite{karunratanakul2020grasping, hasson2019learning} or propose a contact-aware refinement step \cite{yang2021cpf, cao2021reconstructing}. 
More directly related are methods that attempt to generate static grasps given an object and sometimes also  information about the hand \cite{brahmbhatt2019contactdb, brahmbhatt2020contactpose, karunratanakul2021skeletondriven, zhu2021toward, jiang2021graspTTA, karunratanakul2020grasping, taheri2020grabnet}. Generally, these approaches either predict a contact map on the object \cite{brahmbhatt2019contactdb, brahmbhatt2020contactpose, jiang2021graspTTA} or synthesize the joint-angle configuration of the grasping hand \cite{taheri2020grabnet, karunratanakul2020grasping, karunratanakul2021skeletondriven, zhu2021toward}. \cite{jiang2021graspTTA} propose a hybrid method, where predicted contact maps on objects are used to refine an initial grasp prediction. As for RGB-based methods, grasps can be represented as a mesh \cite{taheri2020grabnet, zhu2021toward} or using an implicit surface representation \cite{karunratanakul2020grasping}.
Some methods have combined these two directions, for example by leveraging contact information to post-process noisy hand pose predictions \cite{grady2021contactopt}. \cite{zhang2021manipnet} generate local grasp motions, given the global motion of the hand and object. Similarly, \cite{ye2012synthesis} synthesize hand grasps given full-body and object motions. 
In summary, all of these works focus on generating static grasps and are purely data-driven. In our work, however, we take into consideration the dynamic nature of human-object interaction and consider the physical plausibility of dynamic grasp-based hand-object interactions by leveraging a physics-driven simulation. 

\textbf{Dexterous Hand Control} Different approaches have been used for controlling dexterous hands. 
Learning-based methods most often resort to an anchored hand for in-hand manipulation tasks \cite{openai2018dexterous,huang2021geometry, chen2021simple}, which removes the complexity of generating collision-free trajectories, or rely on expert demonstrations \cite{garciahernando2020iros,christen2019hri,rajeswaran2017rss, qin2021dexmv, hsiao2006imitation}, which can be costly to obtain. \cite{rajeswaran2017rss} collect expert trajectories via teleoperation, which they leverage in an RL setup to learn complex manipulation tasks. \cite{garciahernando2020iros} obtain noisy expert demonstrations from videos and use residual RL to correct the inputs for hand-object interaction tasks. In contrast, we only require a single frame grasp label per sequence. Similar to our work, \cite{christen2019hri} use a parameterized reward function from single data labels for human-robot interactions, but assume a fixed hand to interact with. \cite{jiang2021dash} propose a modular human manipulation framework, but focus on learning power-grasps for picking up objects. \cite{mandikal2020graff} intrinsically motivate a policy to grasp in the affordance region of objects. However, since the policy is only incentivized to grasp in a certain region, the fingers often end up in unnatural configurations. In their follow-up work \cite{mandikal2021dexvip}, the authors address this issue by formulating a reward based on hand-object interaction videos. However, the focus is on a single "consensus" grasp reference per object.  In our work, we propose a method that learns natural object interactions and generates a wider variety of grasps by explicitly conditioning on the desired contact points and hand pose.

\textbf{Physics-aware Inference}
Several recent works have introduced physical awareness to improve purely data-driven approaches \cite{luo2021dynreg,megzhanni2021physshapes,rempe2020eccv,shimada2021neuralcap,shimada2020tog, yuan2021simpoe, ehsani2020force}. \cite{megzhanni2021physshapes} use a physics simulation to validate the plausibility of a generative model for objects via a stability measure. \cite{ehsani2020force} learn to reason about contacts and forces in hand-object interaction videos by leveraging a physics simulation for supervision. To improve the task of human-pose reconstruction from videos, different methods have added physics-based modules to correct the output of a human-pose estimation model. This is achieved either in a post-processing optimization framework \cite{rempe2020eccv,shimada2020tog}, with an approxmation of physics \cite{shimada2021neuralcap}, or via a reinforcement learning policy that directly corrects the pose estimate \cite{yuan2021simpoe}. \cite{luo2021dynreg} regulate a data-driven policy for ego-centric pose estimation with a physics-based policy. They include full-body interactions with larger objects, such as pushing a box.
In contrast to these works, we introduce the novel task of dynamic hand-object interactions, which involves more fine-grained control of the dexterous human hand and has to adhere to the dynamics and displacement of the object of interest. The task also introduces additional complexities due to the increased amount of collision detection queries required for accurately modeling the contacts. To the best of our knowledge, ours is the first method that studies this task and constitutes an important first step into an important direction for human-object interaction. 



==> chapters/04_hoi_generation/dgrasp/sections/tables/table_app_generalization.tex <==
\newcommand{\gclr}{\cellcolor[HTML]{E4E4E4}}
\begin{table*}[ht]
\begin{center}
\resizebox{1.0\linewidth}{!}{
    \begin{tabular}{l|l|c|c|c|c|c|c|c|c|c}
        \toprule
         &   \multicolumn{1}{c}{} & \multicolumn{3}{c|}{GT+PD} & \multicolumn{3}{c|}{GT+IK} & \multicolumn{3}{c}{Ours} \\ \midrule
       & Object  & SimDist [mm/s] $\downarrow$ & Success $\uparrow$  & Interp. [$cm^3$]   & SimDist [mm/s] $\downarrow$ & Success $\uparrow$ & Interp. [$cm^3$] & SimDist [mm/s] $\downarrow$ & Success $\uparrow$ &  Interp. [$cm^3$]\\ \midrule

\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize{Test set 1}}}} 
& \gclr 004 sugar box & \gclr 15.2 $\pm$ 11.4 & \gclr 0.35 & \gclr 5.86 & \gclr 7.4 $\pm$ 9.4 & \gclr 0.60 & \gclr 12.87 & \gclr 2.3 $\pm$ 7.2 & \gclr 0.92 & \gclr 3.35 \\ 
& 005 tomato soup can & 11.4 $\pm$ 10.5 & 0.32 & 4.17 & 11.5 $\pm$ 9.8 & 0.32 & 10.21 & 5.7 $\pm$ 10.3 & 0.76 & 1.56 \\
& \gclr 006 mustard bottle & \gclr 6.0 $\pm$ 8.5 & \gclr 0.60 & \gclr 8.64 & \gclr 2.9 $\pm$ 4.2 & \gclr 0.72 & \gclr 15.44 & \gclr 2.1 $\pm$ 5.7 & \gclr 0.80 & \gclr 1.87 \\ \midrule
& Average & 10.9 $\pm$ 10.1 & 0.42 & 6.22 & 7.3 $\pm$ 7.8 & 0.55 & 12.84 & 3.3 $\pm$ 7.7 & 0.83 & 2.26 \\ \midrule
& & & & & & & & & & \\

\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize{Test set 2}}}} 
& \gclr 061 foam brick & \gclr 18.1 $\pm$ 8.3 & \gclr 0.16 & \gclr 2.06 & \gclr 15.3 $\pm$ 9.9 & \gclr 0.23 & \gclr 5.13 & \gclr 9.6 $\pm$ 12.0 & \gclr 0.62 & \gclr 0.55 \\
& 010 potted meat can & 12.8 $\pm$ 10.2 & 0.33 & 3.80 & 11.3 $\pm$ 10.2 & 0.39 & 8.42 & 5.1 $\pm$ 9.3 & 0.61 & 1.36 \\
& \gclr 052 extra large clamp & \gclr 15.4 $\pm$ 9.6 & \gclr 0.24 & \gclr 2.11 & \gclr 10.3 $\pm$ 10.1 & \gclr 0.44 & \gclr 3.98 & \gclr 14.8 $\pm$ 11.5 & \gclr 0.16 & \gclr 1.53 \\ \midrule
& Average & 15.4 $\pm$ 9.4 & 0.24 & 2.66 & 12.3 $\pm$ 10.1 & 0.35 & 5.84 & 9.8 $\pm$ 10.9 & 0.46 & 1.15 \\ \midrule
& & & & & & & & & & \\

\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize{Test set 3}}}} 
& \gclr 003 cracker box & \gclr 17.4 $\pm$ 10.3 & \gclr 0.20 & \gclr 4.00 & \gclr 9.1 $\pm$ \gclr 10.9 & \gclr 0.52 & \gclr 10.11 & \gclr 12.9 $\pm$ 13.3 & \gclr 0.52 & \gclr 2.86 \\
& 007 tuna fish can & 17.1 $\pm$ 9.4 & 0.14 & 2.28 & 16.5 $\pm$ 9.3 & 0.18 & 4.83 & 5.4 $\pm$ 10.2 & 0.79 & 0.88 \\
& \gclr 011 banana & \gclr 15.8 $\pm$ 9.0 & \gclr 0.11 & \gclr 3.11 & \gclr 14.9 $\pm$ 10.2 & \gclr 0.23 & \gclr 4.78 & \gclr 7.2 $\pm$ 10.3 & \gclr 0.50 & \gclr 1.24 \\ \midrule
& Average & 16.8 $\pm$ 9.6 & 0.15 & 3.13 & 13.5 $\pm$ 10.2 & 0.31 & 6.57 & 8.5 $\pm$ 11.3 & 0.60 & 1.66 \\ \midrule
& & & & & & & & & & \\

\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize{Test set 4}}}} 
& \gclr 002 master chef can & \gclr 18.5 $\pm$ 9.7 & \gclr 0.19 & \gclr 5.33 & \gclr 17.6 $\pm$ 9.7 & \gclr 0.19 & \gclr 12.45 & \gclr 6.6 $\pm$ 11.1 & \gclr 0.65 & \gclr 1.21 \\
& 036 wood block & 15.1 $\pm$ 11.1 & 0.36 & 6.75 & 11.7 $\pm$ 11.7 & 0.50 & 12.98 & 3.4 $\pm$ 8.8 & 0.85 & 3.31 \\
& \gclr 052 extra large clamp & \gclr 15.4 $\pm$ 9.6 & \gclr 0.24 & \gclr 2.11 & \gclr 10.3 $\pm$ 10.1 & \gclr 0.44 & \gclr 3.98 & \gclr 15.1 $\pm$ 11.3 & \gclr 0.28 & \gclr 2.26 \\ \midrule
& Average & 16.3 $\pm$ 10.1 & 0.26 & 4.73 & 13.2 $\pm$ 10.5 & 0.38 & 9.80 & 8.4 $\pm$ 10.4 & 0.59 & 2.26 \\ \midrule
& & & & & & & & & & \\

\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize{Test set 5}}}} 
& \gclr 008 pudding box & \gclr 16.0 $\pm$ 9.4 & \gclr 0.20 & \gclr 3.45 & \gclr 13.0 $\pm$ 11.0 & \gclr 0.38 & \gclr 6.44 & \gclr 3.5 $\pm$ 8.4 & \gclr 0.83 & \gclr 0.90 \\
& 019 pitcher base & 11.4 $\pm$ 11.4 & 0.42 & 7.56 & 11.6 $\pm$ 11.5 & 0.40 & 19.06 & 11.3 $\pm$ 11.5 & 0.40 & 3.52 \\
& \gclr 035 power drill & \gclr 0.6 $\pm$ 1.3 & \gclr 0.87 & \gclr 10.04 & \gclr 4.0 $\pm$ 6.8 & \gclr 0.70 & \gclr 15.57 & \gclr 11.0 $\pm$ 12.8 & \gclr 0.43 & \gclr 1.63 \\ \midrule
& Average & 9.3 $\pm$ 7.4 & 0.50 & 7.02 & 9.6 $\pm$ 9.8 & 0.49 & 13.69 & 8.6 $\pm$ 10.9 & 0.56 & 2.02 \\ \midrule
& & & & & & & & & & \\

\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize{Test set 6}}}} 
& \gclr 005 tomato soup can & \gclr 11.4 $\pm$ 10.5 & \gclr 0.32 & \gclr 4.17 & \gclr 11.5 $\pm$ 9.8 & \gclr 0.32 & \gclr 10.21 & \gclr 9.1 $\pm$ 12.0 & \gclr 0.60 & \gclr 2.10 \\
& 037 scissors & 9.9 $\pm$ 9.9 & 0.39 & 2.55 & 11.3 $\pm$ 9.2 & 0.31 & 4.11 & 18.3 $\pm$ 10.4 & 0.19 & 0.71 \\
& \gclr 040 large marker & \gclr 19.6 $\pm$ 5.3 & \gclr 0.03 & \gclr 1.38 & \gclr 20.0 $\pm$ 6.4 & \gclr 0.07 & \gclr 2.95 & \gclr 18.2 $\pm$ 10.2 & \gclr 0.19 & \gclr 0.51 \\  \midrule
& Average & 13.6 $\pm$ 8.6 & 0.25 & 2.70 & 14.3 $\pm$ 8.4 & 0.23 & 5.76 & 15.2 $\pm$ 10.9 & 0.33 & 1.11 \\ \bottomrule

\end{tabular}}
\end{center}
\caption{\textbf{Generalization to Unseen Objects}. We evaluate generalization to unseen objects and compare our model with the baselines. We create six different test sets of three objects, which we leave out during training. We report the detailed results per test set in this table. }
\label{tab:app_generalization}
\end{table*}

==> chapters/04_hoi_generation/dgrasp/sections/tables/table_app_policies.tex <==
\begin{table}[t]
	\centering
	\resizebox{\columnwidth}{!}{%
		\begin{tabular}{ll|ccc}
		
			\toprule
            
			& Models & Success $\uparrow$ & SimDist [mm/s] $\downarrow$ & Interpenetration $\downarrow$ \\ \midrule
			
			\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Train}}}
            &  Ours PO & \textbf{0.81}  & $\mathbf{3.7 \pm 5.8}$ & 1.94 \\
            & \greycellcol Ours AO & \greycellcol 0.7  & \greycellcol $5.8 \pm 7.4$ &  \greycellcol \textbf{1.75} \\ \midrule

            
			\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Test}}}
            & Ours PO & 0.42 & $12.4 \pm 10.4$ & \textbf{1.19} \\
            & \greycellcol Ours AO & \greycellcol \textbf{0.63}  & \greycellcol $\mathbf{8.0 \pm 8.1}$ &  \greycellcol 1.77 \\
			\bottomrule
		\end{tabular}%
	}

	\caption{\textbf{Policy Type Comparison}. We compare a single policy trained over multiple objects (Ours AO) and single policies trained per object (Ours PO). We find that the all-object policies lead to better generalization performance on the DexYCB dataset \cite{chao2021dexycb}.}
	\label{tab:app_policies}
\end{table}



==> chapters/04_hoi_generation/dgrasp/sections/tables/table_contactopt_test.tex <==
\begin{table*}[t]
\begin{center}
\resizebox{0.8\linewidth}{!}{
    \begin{tabular}{@{}l|c|c|c|c|c|c}
        \toprule
            \multicolumn{1}{c}{} & \multicolumn{3}{c|}{Grady \textit{et. al} \cite{grady2021contactopt}+PD} & \multicolumn{3}{c}{Ours} \\ \midrule
        Object  & SimDist [mm/s] $\downarrow$ & Success $\uparrow$  & Interp. [$cm^3$]   & SimDist [mm/s] $\downarrow$ & Success $\uparrow$ &  Interp. [$cm^3$]\\ \midrule
\rowcolor{Gray}
003 cracker box & 6.7 $\pm$ 9.7 & 0.60 & 13.41 & 0.26 $\pm$ 0.1 & 1.00 & 2.14 \\
004 sugar box & 23.6 $\pm$ 1.5 & 0.00 & 17.71 & 0.95 $\pm$ 2.2 & 0.90 & 2.53 \\
\rowcolor{Gray}
006 mustard bottle & 4.6 $\pm$ 7.6 & 0.60 & 25.16 & 0.64 $\pm$ 0.8 & 0.80 & 2.46 \\
010 potted meat can & 1.9 $\pm$ 5.5 & 0.90 & 14.08 & 0.63 $\pm$ 1.3 & 0.90 & 0.38 \\
\rowcolor{Gray}
011 banana & 12.0 $\pm$ 10.4 & 0.20 & 13.38 & 0.61 $\pm$ 0.5 & 0.80 & 1.91 \\
021 bleach cleanser & 0.9 $\pm$ 2.4 & 0.90 & 18.23 & 2.86 $\pm$ 7.6 & 0.90 & 2.25 \\
\rowcolor{Gray}
025 mug & 6.4 $\pm$ 8.4 & 0.50 & 4.80 & 5.05 $\pm$ 9.7 & 0.80 & 4.16 \\
035 power drill & 0.1 $\pm$ 0.1 & 1.00 & 14.84 & 0.71 $\pm$ 0.6 & 0.60 & 1.68 \\
\rowcolor{Gray}
037 scissors & 2.7 $\pm$ 6.9 & 0.70 & 4.34 & 5.30 $\pm$ 9.3 & 0.60 & 1.21 \\
\midrule
Average & 6.5 $\pm$ 5.8 & 0.60 & 13.99 & 1.9 $\pm$ 3.57 & 0.81 & 2.08 \\ \bottomrule
    \end{tabular}}
\end{center}
\caption{Detailed results for the test set with ContactOpt \cite{grady2021contactopt} on HO3D images.}
\label{tab:exp1_test_contactopt_full}
\end{table*}

==> chapters/04_hoi_generation/dgrasp/sections/tables/table_contactopt_train.tex <==
\begin{table*}[t]
\begin{center}
\resizebox{0.8\linewidth}{!}{
    \begin{tabular}{@{}l|c|c|c|c|c|c}
        \toprule
            \multicolumn{1}{c}{} & \multicolumn{3}{c|}{Grady \textit{et. al} \cite{grady2021contactopt}+PD} & \multicolumn{3}{c}{Ours} \\ \midrule
        Object  & SimDist [mm/s] $\downarrow$ & Success $\uparrow$  & Interp. [$cm^3$]   & SimDist [mm/s] $\downarrow$ & Success $\uparrow$ &  Interp. [$cm^3$]\\ \midrule
\rowcolor{Gray}
003 cracker box & 2.5 $\pm$ 6.7 & 0.85 & 14.33 & 0.3 $\pm$ 0.1 & 1.00 & 3.18 \\
004 sugar box & 16.3 $\pm$ 9.3 & 0.05 & 17.04 & 2.9 $\pm$ 6.6 & 0.70 & 2.40 \\
\rowcolor{Gray}
006 mustard bottle & 9.1 $\pm$ 9.7 & 0.40 & 26.46 & 0.3 $\pm$ 0.4 & 0.95 & 2.89 \\
010 potted meat can & 3.9 $\pm$ 8.5 & 0.70 & 15.42 & 2.2 $\pm$ 5.9 & 0.90 & 0.78 \\
\rowcolor{Gray}
011 banana & 10.0 $\pm$ 9.9 & 0.35 & 13.80 & 1.7 $\pm$ 4.9 & 0.80 & 1.98 \\
021 bleach cleanser & 0.9 $\pm$ 3.3 & 0.95 & 18.84 & 0.3 $\pm$ 0.1 & 1.00 & 2.86 \\
\rowcolor{Gray}
025 mug & 2.7 $\pm$ 6.7 & 0.80 & 5.49 & 2.0 $\pm$ 5.4 & 0.85 & 4.74 \\
035 power drill & 0.2 $\pm$ 0.4 & 0.95 & 16.09 & 0.3 $\pm$ 0.2 & 1.00 & 2.56 \\
\rowcolor{Gray}
037 scissors & 0.1 $\pm$ 0.1 & 1.00 & 6.96 & 3.0 $\pm$ 7.3 & 0.75 & 2.60 \\
\midrule
Average & 5.1 $\pm$ 6.1 & 0.67 & 14.94 & 1.4 $\pm$ 3.4 & 0.88 & 2.67 \\ \bottomrule
    \end{tabular}}
\end{center}
\caption{Detailed results for the train set with ContactOpt \cite{grady2021contactopt} on HO3D images.}
\label{tab:exp1_train_contactopt_full}
\end{table*}

==> chapters/04_hoi_generation/dgrasp/sections/tables/table_exp1.tex <==
\newcommand{\greycellcol}{\cellcolor[HTML]{E4E4E4}}
\begin{table*}[t]
	\centering
	\resizebox{2\columnwidth}{!}{%
		\begin{tabular}{ll|ccc|ccc}
		
			\toprule
            & \multirow{2}{*}{Models} & \multicolumn{3}{c}{Training set} & \multicolumn{3}{c}{Test set} \\
			&  & Success [\%] $\uparrow$ & SimDist [mm/s] $\downarrow$ & Interp. [$cm^3$] $\downarrow$ & Success [\%] $\uparrow$ & SimDist [mm/s] $\downarrow$ & Interp. [$cm^3$] $\downarrow$  \\
			
			\midrule

			\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{DexYCB}}}  
			& GT+PD & 0.2 & $15.8 \pm 7.9$ & 0.38 & 0.23 & 15.6 $\pm 6.6$ & 0.78 \\
% 			\rowcolor{Gray}
% 			& GraspTTA \cite{jiang2021graspTTA} & & \\
            & \greycellcol GT+IK & \greycellcol 0.25 & \greycellcol $14.8 \pm 9.1$ & \greycellcol 0.74 & \greycellcol 0.35 & \greycellcol $13.2 \pm 9.1 $ & \greycellcol 1.41\\
            
            
            & \textbf{Ours} & \textbf{0.81}  & $3.7 \pm 5.8$  & \textbf{0.10} & 0.42  & $12.4 \pm 10.4$  & \textbf{0.14}\\
            
            & \greycellcol Ours AllObj & \greycellcol 0.73 & \greycellcol $\mathbf{3.0 \pm 5.5}$ & \greycellcol - & \greycellcol \textbf{0.6} & \greycellcol $\mathbf{4.8 \pm 6.7}$ & \greycellcol -\\

			%\rowcolor{Gray}

			
			\midrule
			
		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{DexYCB}}} 
			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+PD & 0.25 & $12.6 \pm 6.5$ &  5.35 & 0.25 & $13.0 \pm 7.3 $ &  5.31 \\
			
			& \greycellcol Jiang \textit{et. al} \cite{jiang2021graspTTA}+IK & \greycellcol 0.29 & \greycellcol $14.9 \pm 10.1$ & \greycellcol 0.57 & \greycellcol 0.30 & \greycellcol $12.5 \pm 8.7 $ & \greycellcol 6.42 \\
			
			& \textbf{Ours} & 0.60 & $\mathbf{5.2 \pm 6.5}$ & \textbf{0.05} & 0.44 & 7.7 \pm 7.5 & \textbf{0.08} \\
			& \greycellcol \textbf{Ours corrected} & \greycellcol  \textbf{0.80} &  \greycellcol $\mathbf{2.2 \pm 4.6}$ & \greycellcol - & \greycellcol \textbf{0.68} & \greycellcol $\mathbf{4.0 \pm 5.8}$ & \greycellcol - \\
% 			\cmidrule(lr){2-11}
			% \rowcolor{Gray}

			
			\midrule
			
		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{HO3D}}} 
			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+PD & 0.28 & $ 11.5 \pm 6.6$ & 2.82 & 0.28 & $11.9 \pm 8.6 $ & 2.85\\
			& \greycellcol Jiang \textit{et. al} \cite{jiang2021graspTTA}+IK & \greycellcol 0.29 & \greycellcol $13.2 \pm 9.4$ & \greycellcol 6.51 & \greycellcol 0.34 & \greycellcol $10.6 \pm 8.0 $ & \greycellcol 0.51 \\
			& \textbf{Ours} & 0.61 & 5.5 \pm 6.5 & \textbf{0.03} & 0.39 & 8.6 \pm 7.8 & \textbf{0.06} \\
			& \greycellcol \textbf{Ours corrected} & \greycellcol  \textbf{0.77} &  \greycellcol $\mathbf{2.7 \pm 5.9}$ & \greycellcol - & \greycellcol \textbf{0.66} & \greycellcol $\mathbf{5.5 \pm 7.4}$ & \greycellcol - \\
% 			\cmidrule(lr){2-11}
			% \rowcolor{Gray}
			
			\bottomrule
			
		\end{tabular}%
	}
	% \vspace{2mm}
	\caption{\textbf{Static grasp evaluation}. 
	We compare our model with grasp samples from the DexYCB dataset (top row) or generated by a grasp synthesis method (middle and bottom row). We evaluate the baseline grasps in the simulation via PD-control (*+PD) directly or after de-noising via inverse kinematics (*+IK). \update{We observe that our method outperforms the baselines on both the training and test sets on all the metrics. The results indicate that static grasp references 1) will not lead to stable grasps when evaluated in a physics simulation and 2) suffer from interpenetration. Our method can correct the interpenetration and learn stable grasps in a dynamic setting.}
	}
	\label{tab:exp1_train}
\end{table*}{}

% \begin{table*}[]
% 	\centering
% 	\resizebox{2\columnwidth}{!}{%
% 		\begin{tabular}{lc|ccc|ccc}
		
% 			\toprule
%             & \multirow{2}{*}{Models} & \multicolumn{3}{c}{Training set} & \multicolumn{3}{c}{Testing set} \\
% 			&  & Success [\%] $\uparrow$ & SimDist [mm] $\downarrow$ & Interp. [mm] $\downarrow$ & Success [\%] $\uparrow$ & SimDist [mm] $\downarrow$ & Interp. [mm] $\downarrow$  \\
			
% 			\midrule

% 			\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{DexYCB}}}  
% 			& GT+PD & 0.2 & $15.8 \pm 7.9$ & tbd & 0.23 & 15.6 $\pm 6.6$ & tbd \\
% % 			\rowcolor{Gray}
% % 			& GraspTTA \cite{jiang2021graspTTA} & & \\
%             & \cellcolor[HTML]{E4E4E4}GT+IK & \cellcolor[HTML]{E4E4E4}0.25 & \cellcolor[HTML]{E4E4E4}$14.8 \pm 9.1$ & \cellcolor[HTML]{E4E4E4}tbd & \cellcolor[HTML]{E4E4E4}0.35 & \cellcolor[HTML]{E4E4E4}$13.2 \pm 9.1 $ & \cellcolor[HTML]{E4E4E4}tbd\\
            
            
%             & Ours & \textbf{0.81}  & $\mathbf{3.7 \pm 5.8}$  & \textbf{0} & \textbf{0.42}  & $\mathbf{12.4 \pm 10.4}$  & \textbf{0}\\

% 			%\rowcolor{Gray}

			
% 			\midrule
			
% 		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{DexYCB}}} 
% 			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+PD & 0.25 & $12.6 \pm 6.5$ & tbd & 0.25 & $13.0 \pm 7.3 $ & tbd \\
% 			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+IK & 0.29 & $14.9 \pm 10.1$ & tbd & 0.30 & $12.5 \pm 8.7 $ & tbd \\
% 			& Ours & \textbf{0.60} & $\mathbf{5.2 \pm 6.5}$ & \textbf{0} & \textbf{0.44} & $\mathbf{7.7 \pm 7.5}$ & \textbf{0} \\
% % 			\cmidrule(lr){2-11}
% 			% \rowcolor{Gray}

			
% 			\midrule
			
% 		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{HO3D}}} 
% 			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+PD & 0.28 & $ 11.5 \pm 6.6$ & tbd & 0.28 & $11.9 \pm 8.6 $ & tbd\\
% 			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+IK & 0.29 & $ 13.2 \pm 9.4$ & tbd & 0.34 & $10.6 \pm 8.0 $ & tbd \\
% 			& Ours & \textbf{0.61} & $\mathbf{5.5 \pm 6.5}$ & \textbf{0} & \textbf{0.39} & $\mathbf{8.6 \pm 7.8}$ & \textbf{0} \\
% % 			\cmidrule(lr){2-11}
% 			% \rowcolor{Gray}
			
% 			\bottomrule
			
% 		\end{tabular}%
% 	}
% 	% \vspace{2mm}
% 	\caption{Evaluation on train and test set}
% 	\label{tab:exp1_train}
% \end{table*}{}



% \begin{table}[]
% 	\centering
% 	\resizebox{\columnwidth}{!}{%
% 		\begin{tabular}{lc|ccc}
		
% 			\toprule

% 			& Models & Success [\%] $\uparrow$ & SimDist [mm] $\downarrow$ & Interp. [mm] $\downarrow$  \\
			
% 			\midrule

% 			\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{DexYCB}}}  
% 			& GT+PD & 0.23 & 15.6 $\pm 6.6$ & tbd\\
% % 			\rowcolor{Gray}
% % 			& GraspTTA \cite{jiang2021graspTTA} & & \\
%             & GT+IK & 0.35 & $13.2 \pm 9.1 $ & tbd\\
            
%             & Ours & \textbf{0.42}  & $\mathbf{12.4 \pm 10.4}$  & \textbf{0}\\

% % 			\rowcolor{Gray}

			
% 			\midrule
			
% 		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{DexYCB}}} 
% 			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+PD & 0.25 & $13.0 \pm 7.3 $ & tbd \\
% 			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+IK & 0.30 & $12.5 \pm 8.7 $ & tbd  \\
% 			& Ours & \textbf{0.44} & $\mathbf{7.7 \pm 7.5}$ & \textbf{0}\\
% % 			\cmidrule(lr){2-11}
% 			% \rowcolor{Gray}

% 					\midrule
			
% 		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{HO3D}}} 
% 			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+PD & 0.28 & $11.9 \pm 8.6 $ & tbd \\
% 			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+IK & 0.34 & $10.6 \pm 8.0 $ & tbd \\
% 			& Ours & \textbf{0.39} & $\mathbf{8.6 \pm 7.8}$ & \textbf{0}\\
% % 			\cmidrule(lr){2-11}
% 			% \rowcolor{Gray}
			
% 			\bottomrule
			
% 		\end{tabular}%
% 	}
% 	% \vspace{2mm}
% 	\caption{Evaluation on test set}
% 	\label{tab:exp1_test}
% \end{table}{}

==> chapters/04_hoi_generation/dgrasp/sections/tables/table_exp1_gen.tex <==
\begin{table}[t]
	\centering
	\resizebox{0.7\columnwidth}{!}{%
		\begin{tabular}{l|ccc}
		
			\toprule

			Models & Success $\uparrow$ & SimDist [mm/s] $\downarrow$ & Interpenetration [$cm^3$]$\downarrow$  \\
			
			\midrule
            GT+PD & 0.30 & $13.7 \pm 9.2$ & 4.41 \\
            \rowcolor{Gray}
            GT+IK & 0.38 & $11.7 \pm 9.4$ & 9.08 \\
            \textbf{Ours} & \textbf{0.56} & $\mathbf{9.0 \pm 10.4}$ & \textbf{1.74}\\
			
			\bottomrule
		\end{tabular}%
	}
    \vspace{-0.1cm}
	\caption{\textbf{Generalization}. We evaluate generalization to unseen objects and compare our model with the baselines. We create six different test sets of three objects each, which we leave out during training. We report the average performance over all test sets. %Our method outperforms the baseline, however, leaving room for improvement for future work.
	}
	\label{tab:exp1_gen}
\end{table}{}



==> chapters/04_hoi_generation/dgrasp/sections/tables/table_exp1_test.tex <==
\begin{table}[]
	\centering
	\resizebox{\columnwidth}{!}{%
		\begin{tabular}{lc|ccc}
		
			\toprule

			& Models & Success [\%] $\uparrow$ & SimDist [mm] $\downarrow$ & Interp. [mm] $\downarrow$  \\
			
			\midrule

			\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{DexYCB}}}  
			& GT+PD & 0.23 & 15.6 $\pm 6.6$ & tbd\\
% 			\rowcolor{Gray}
% 			& GraspTTA \cite{jiang2021graspTTA} & & \\
            & GT+IK & 0.35 & $13.2 \pm 9.1 $ & tbd\\
            
            & Ours & \textbf{0.42}  & $\mathbf{12.4 \pm 10.4}$  & \textbf{0}\\

% 			\rowcolor{Gray}

			
			\midrule
			
		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{DexYCB}}} 
			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+PD & 0.25 & $13.0 \pm 7.3 $ & tbd \\
			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+IK & 0.30 & $12.5 \pm 8.7 $ & tbd  \\
			& Ours & \textbf{0.44} & $\mathbf{7.7 \pm 7.5}$ & \textbf{0}\\
% 			\cmidrule(lr){2-11}
			% \rowcolor{Gray}

					\midrule
			
		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{HO3D}}} 
			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+PD & 0.28 & $11.9 \pm 8.6 $ & tbd \\
			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+IK & 0.34 & $10.6 \pm 8.0 $ & tbd \\
			& Ours & \textbf{0.39} & $\mathbf{8.6 \pm 7.8}$ & \textbf{0}\\
% 			\cmidrule(lr){2-11}
			% \rowcolor{Gray}
			
			\bottomrule
			
		\end{tabular}%
	}
	% \vspace{2mm}
	\caption{Evaluation on test set}
	\label{tab:exp1_test}
\end{table}{}



==> chapters/04_hoi_generation/dgrasp/sections/tables/table_exp1_test_full.tex <==
\begin{table*}[t]
\begin{center}
\resizebox{0.8\linewidth}{!}{
    \begin{tabular}{@{}l|c|c|c|c|c|c|c|c|c}
        \toprule
            \multicolumn{1}{c}{} & \multicolumn{3}{c|}{GT+PD} & \multicolumn{3}{c|}{GT+IK} & \multicolumn{3}{c}{Ours} \\ \midrule
        Object  & SimDist [mm/s] $\downarrow$ & Success $\uparrow$  & Interp. [$cm^3$]   & SimDist [mm/s] $\downarrow$ & Success  $\uparrow$ & Interp. [$cm^3$] & SimDist [mm/s] $\downarrow$ & Success $\uparrow$ &  Interp. [$cm^3$]\\ \midrule
002 master chef can & 20.4 $\pm$ 9.3 & 0.17 & 4.17 & 19.2 $\pm$ 8.6 & 0.17 & 10.73 & 0.6 $\pm$ 1.2 & 0.83 & 1.67 \\
\rowcolor{Gray}
003 cracker box & 14.7 $\pm$ 11.1 & 0.33 & 5.21 & 9.0 $\pm$ 11.5 & 0.67 & 13.10 & 8.9 $\pm$ 12.4 & 0.67 & 4.06 \\
004 sugar box & 14.1 $\pm$ 12.1 & 0.43 & 6.75 & 3.9 $\pm$ 8.5 & 0.86 & 16.04 & 3.9 $\pm$ 9.3 & 0.86 & 3.02 \\
\rowcolor{Gray}
005 tomato soup can & 7.6 $\pm$ 9.0 & 0.50 & 3.25 & 8.2 $\pm$ 8.4 & 0.25 & 7.56 & 14.4 $\pm$ 11.4 & 0.25 & 1.03 \\
006 mustard bottle & 9.5 $\pm$ 9.9 & 0.50 & 6.77 & 6.7 $\pm$ 9.9 & 0.63 & 13.19 & 7.0 $\pm$ 12.0 & 0.75 & 2.13 \\
\rowcolor{Gray}
007 tuna fish can & 16.4 $\pm$ 9.4 & 0.14 & 1.55 & 16.3 $\pm$ 8.5 & 0.14 & 3.55 & 0.1 $\pm$ 0.0 & 1.00 & 1.50 \\
008 pudding box & 18.5 $\pm$ 8.2 & 0.17 & 2.08 & 12.7 $\pm$ 10.5 & 0.33 & 4.19 & 4.2 $\pm$ 9.2 & 0.83 & 0.92 \\
\rowcolor{Gray}
009 gelatin box & 21.6 $\pm$ 9.7 & 0.14 & 2.00 & 15.3 $\pm$ 13.3 & 0.29 & 4.59 & 3.8 $\pm$ 8.5 & 0.71 & 0.86 \\
010 potted meat can & 9.9 $\pm$ 10.2 & 0.40 & 2.60 & 10.8 $\pm$ 10.8 & 0.40 & 7.00 & 0.1 $\pm$ 0.1 & 1.00 & 1.00 \\
\rowcolor{Gray}
011 banana & 13.8 $\pm$ 9.9 & 0.14 & 2.79 & 13.0 $\pm$ 10.8 & 0.29 & 4.36 & 10.8 $\pm$ 12.0 & 0.43 & 0.50 \\
019 pitcher base & 12.6 $\pm$ 12.5 & 0.50 & 7.83 & 13.1 $\pm$ 12.7 & 0.50 & 25.54 & 6.2 $\pm$ 9.1 & 0.50 & 3.08 \\
\rowcolor{Gray}
021 bleach cleanser & 5.8 $\pm$ 8.3 & 0.40 & 10.43 & 5.1 $\pm$ 9.3 & 0.80 & 15.40 & 10.2 $\pm$ 12.3 & 0.60 & 2.10 \\
024 bowl & 9.3 $\pm$ 11.1 & 0.50 & 5.83 & 0.3 $\pm$ 0.3 & 1.00 & 13.44 & 12.0 $\pm$ 11.9 & 0.50 & 1.56 \\
\rowcolor{Gray}
025 mug & 7.4 $\pm$ 9.2 & 0.50 & 3.00 & 0.5 $\pm$ 0.5 & 1.00 & 9.13 & 4.1 $\pm$ 9.0 & 0.83 & 1.33 \\
035 power drill & 0.2 $\pm$ 0.1 & 1.00 & 8.25 & 0.5 $\pm$ 0.4 & 0.83 & 15.02 & 5.6 $\pm$ 10.4 & 0.67 & 2.71 \\
\rowcolor{Gray}
036 wood block & 20.6 $\pm$ 9.1 & 0.17 & 4.88 & 12.9 $\pm$ 12.4 & 0.50 & 11.73 & 0.2 $\pm$ 0.1 & 1.00 & 4.17 \\
037 scissors & 8.1 $\pm$ 9.9 & 0.50 & 4.44 & 6.4 $\pm$ 8.6 & 0.50 & 6.55 & 19.0 $\pm$ 8.1 & 0.13 & 0.58 \\
\rowcolor{Gray}
040 large marker & 18.7 $\pm$ 3.2 & 0.00 & 1.43 & 13.5 $\pm$ 8.7 & 0.20 & 3.58 & 24.2 $\pm$ 0.1 & 0.00 & 0.00 \\
052 extra large clamp & 16.2 $\pm$ 8.9 & 0.14 & 2.48 & 5.1 $\pm$ 7.7 & 0.43 & 5.21 & 14.0 $\pm$ 12.1 & 0.43 & 1.88 \\
\rowcolor{Gray}
061 foam brick & 16.0 $\pm$ 10.8 & 0.29 & 2.43 & 10.0 $\pm$ 8.3 & 0.13 & 4.86 & 10.5 $\pm$ 12.0 & 0.57 & 1.30 \\  \midrule
Average & 13.1 $\pm$ 9.1 & 0.35 & 4.41 & 9.1 $\pm$ 8.5 & 0.50 & 9.74 & 8.0 $\pm$ 8.1 & 0.63 & 1.77 \\ \bottomrule
    \end{tabular}}
\end{center}
\caption{Detailed results for the DexYCB test set.}
\label{tab:exp1_test_full}
\end{table*}

  

==> chapters/04_hoi_generation/dgrasp/sections/tables/table_exp1_train.tex <==
\begin{table}[]
	\centering
	\resizebox{\columnwidth}{!}{%
		\begin{tabular}{lc|ccc}
		
			\toprule

			& Models & Success [\%] $\uparrow$ & SimDist [mm] $\downarrow$ & Interp. [mm] $\downarrow$  \\
			
			\midrule

			\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{DexYCB}}}  
			& GT+PD & 0.2 & $15.8 \pm 7.9$ & tbd\\
			%\rowcolor{Gray}
% 			& GraspTTA \cite{jiang2021graspTTA} & & \\
            & GT+IK & 0.25 & $14.8 \pm 9.1$ & tbd\\
            
            & Ours & \textbf{0.81}  & $\mathbf{3.7 \pm 5.8}$  & \textbf{0}\\

			%\rowcolor{Gray}

			
			\midrule
			
		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{DexYCB}}} 
			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+PD & 0.25 & $12.6 \pm 6.5$ & tbd \\
			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+IK & 0.29 & $14.9 \pm 10.1$ & tbd \\
			& Ours & \textbf{0.60} & $\mathbf{5.2 \pm 6.5}$ & \textbf{0} \\
% 			\cmidrule(lr){2-11}
			% \rowcolor{Gray}

			
			\midrule
			
		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{HO3D}}} 
			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+PD & 0.28 & $ 11.5 \pm 6.6$ & tbd \\
			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+IK & 0.29 & $ 13.2 \pm 9.4$ & tbd  \\
			& Ours & \textbf{0.61} & $\mathbf{5.5 \pm 6.5}$ & \textbf{0} \\
% 			\cmidrule(lr){2-11}
			% \rowcolor{Gray}
			
			\bottomrule
			
		\end{tabular}%
	}
	% \vspace{2mm}
	\caption{Evaluation on train set}
	\label{tab:dgrasp:exp1_train}
\end{table}{}



==> chapters/04_hoi_generation/dgrasp/sections/tables/table_exp1_train_full.tex <==
\begin{table*}[ht]
\begin{center}
\resizebox{0.8\linewidth}{!}{
    \begin{tabular}{@{}l|c|c|c|c|c|c|c|c|c}
        \toprule
            \multicolumn{1}{c}{} & \multicolumn{3}{c|}{GT+PD} & \multicolumn{3}{c|}{GT+IK} & \multicolumn{3}{c}{Ours} \\ \midrule
        Object  & SimDist [mm/s] $\downarrow$ & Success $\uparrow$  & Interp. [$cm^3$]   & SimDist [mm/s] $\downarrow$ & Success $\uparrow$ & Interp. [$cm^3$] & SimDist [mm/s] $\downarrow$ & Success $\uparrow$ &  Interp. [$cm^3$]\\ \midrule
002 master chef can & 18.0 $\pm$ 9.8 & 0.19 & 5.68 & 17.2 $\pm$ 10.0 & 0.20 & 12.96 & 1.5 $\pm$ 5.7 & 0.90 & 1.54 \\
\rowcolor{Gray}
003 cracker box & 18.2 $\pm$ 10.1 & 0.16 & 3.62 & 9.2 $\pm$ 10.7 & 0.47 & 9.16 & 8.4 $\pm$ 12.3 & 0.68 & 2.48 \\
004 sugar box & 15.6 $\pm$ 11.2 & 0.32 & 5.52 & 8.7 $\pm$ 9.7 & 0.50 & 11.64 & 0.1 $\pm$ 0.0 & 1.00 & 3.28 \\
\rowcolor{Gray}
005 tomato soup can & 12.1 $\pm$ 10.8 & 0.28 & 4.34 & 12.2 $\pm$ 10.1 & 0.33 & 10.72 & 1.4 $\pm$ 5.5 & 0.90 & 2.51 \\
006 mustard bottle & 4.4 $\pm$ 7.8 & 0.64 & 9.51 & 1.1 $\pm$ 1.5 & 0.76 & 16.50 & 3.2 $\pm$ 8.5 & 0.88 & 2.20 \\
\rowcolor{Gray}
007 tuna fish can & 17.4 $\pm$ 9.4 & 0.14 & 2.52 & 16.6 $\pm$ 9.6 & 0.19 & 5.26 & 1.8 $\pm$ 4.6 & 0.71 & 1.13 \\
008 pudding box & 15.1 $\pm$ 9.7 & 0.21 & 3.91 & 13.2 $\pm$ 11.2 & 0.39 & 7.19 & 2.4 $\pm$ 5.9 & 0.78 & 0.98 \\
\rowcolor{Gray}
009 gelatin box & 18.9 $\pm$ 9.4 & 0.15 & 2.23 & 18.3 $\pm$ 9.3 & 0.20 & 4.61 & 3.7 $\pm$ 8.6 & 0.85 & 0.98 \\
010 potted meat can & 13.6 $\pm$ 10.3 & 0.30 & 4.14 & 11.4 $\pm$ 10.0 & 0.39 & 8.81 & 1.8 $\pm$ 6.0 & 0.89 & 0.64 \\
\rowcolor{Gray}
011 banana & 16.7 $\pm$ 8.6 & 0.09 & 3.27 & 15.9 $\pm$ 10.0 & 0.20 & 4.97 & 5.9 $\pm$ 9.6 & 0.47 & 0.73 \\
019 pitcher base & 11.0 $\pm$ 11.1 & 0.40 & 7.47 & 11.2 $\pm$ 11.2 & 0.37 & 17.01 & 6.9 $\pm$ 10.8 & 0.68 & 3.16 \\
\rowcolor{Gray}
021 bleach cleanser & 5.1 $\pm$ 8.5 & 0.61 & 8.25 & 3.8 $\pm$ 7.0 & 0.61 & 15.64 & 0.2 $\pm$ 0.4 & 0.94 & 3.08 \\
024 bowl & 10.2 $\pm$ 10.7 & 0.41 & 3.15 & 7.3 $\pm$ 9.3 & 0.62 & 9.83 & 7.5 $\pm$ 10.7 & 0.62 & 2.08 \\
\rowcolor{Gray}
025 mug & 12.3 $\pm$ 10.3 & 0.35 & 3.24 & 9.7 $\pm$ 10.6 & 0.53 & 6.56 & 10.2 $\pm$ 12.2 & 0.59 & 1.61 \\
035 power drill & 0.8 $\pm$ 1.8 & 0.83 & 10.68 & 5.3 $\pm$ 9.0 & 0.65 & 15.76 & 6.4 $\pm$ 10.7 & 0.59 & 1.64 \\
\rowcolor{Gray}
036 wood block & 13.4 $\pm$ 11.6 & 0.42 & 7.31 & 11.3 $\pm$ 11.5 & 0.50 & 13.36 & 0.1 $\pm$ 0.0 & 1.00 & 3.56 \\
037 scissors & 10.6 $\pm$ 9.9 & 0.35 & 1.72 & 13.5 $\pm$ 9.4 & 0.22 & 3.03 & 19.3 $\pm$ 10.0 & 0.11 & 0.35 \\
\rowcolor{Gray}
040 large marker & 19.8 $\pm$ 5.8 & 0.04 & 1.38 & 21.5 $\pm$ 5.9 & 0.05 & 2.81 & 20.9 $\pm$ 7.3 & 0.05 & 0.09 \\
052 extra large clamp & 15.0 $\pm$ 9.9 & 0.28 & 1.97 & 12.3 $\pm$ 11.0 & 0.44 & 3.50 & 10.4 $\pm$ 11.7 & 0.44 & 1.70 \\
\rowcolor{Gray}
061 foam brick & 18.9 $\pm$ 7.3 & 0.12 & 1.93 & 17.2 $\pm$ 10.5 & 0.26 & 5.23 & 3.5 $\pm$ 8.1 & 0.84 & 1.30 \\
\midrule
Average & 13.4 $\pm$ 9.2 & 0.31 & 4.59 & 11.8 $\pm$ 9.4 & 0.39 & 9.23 & 5.8 $\pm$ 7.4 & 0.70 & 1.75 \\ \bottomrule
    \end{tabular}}
\end{center}
\vspace{-0.2cm}
\caption{Detailed results for the DexYCB train set.}
\label{tab:exp1_train_full}
\end{table*}



==> chapters/04_hoi_generation/dgrasp/sections/tables/table_gtta_test.tex <==
\begin{table*}[t]
\begin{center}
\resizebox{0.8\linewidth}{!}{
    \begin{tabular}{@{}l|c|c|c|c|c|c|c|c|c}
        \toprule
            \multicolumn{1}{c}{} & \multicolumn{3}{c|}{Jiang \textit{et. al} \cite{jiang2021graspTTA}+PD} & \multicolumn{3}{c|}{Jiang \textit{et. al} \cite{jiang2021graspTTA}+IK} & \multicolumn{3}{c}{Ours} \\ \midrule
        Object  & SimDist [mm/s] $\downarrow$ & Success $\uparrow$  & Interp. [$cm^3$]   & SimDist [mm/s] $\downarrow$ & Success $\uparrow$ & Interp. [$cm^3$] & SimDist [mm/s] $\downarrow$ & Success $\uparrow$ &  Interp. [$cm^3$]\\ \midrule
002 master chef can & 24.0 $\pm$ 1.6 & 0.00 & 7.54 & 23.3 $\pm$ 1.3 & 0.00 & 7.03 & 5.3 $\pm$ 10.5 & 0.80 & 1.88 \\
\rowcolor{Gray}
003 cracker box* & 22.8 $\pm$ 2.5 & 0.00 & 6.73 & 20.3 $\pm$ 5.4 & 0.00 & 7.74 & 5.4 $\pm$ 10.6 & 0.80 & 7.06 \\
004 sugar box* & 15.2 $\pm$ 8.7 & 0.10 & 5.18 & 15.0 $\pm$ 8.4 & 0.00 & 13.85 & 0.2 $\pm$ 0.2 & 1.00 & 3.48 \\
\rowcolor{Gray}
005 tomato soup can & 14.6 $\pm$ 9.0 & 0.10 & 5.29 & 15.0 $\pm$ 9.0 & 0.00 & 10.75 & 0.1 $\pm$ 0.1 & 1.00 & 5.86 \\
006 mustard bottle* & 5.2 $\pm$ 7.3 & 0.50 & 5.19 & 7.6 $\pm$ 7.6 & 0.10 & 14.29 & 0.4 $\pm$ 0.9 & 0.90 & 6.23 \\
\rowcolor{Gray}
007 tuna fish can & 21.4 $\pm$ 1.7 & 0.00 & 2.61 & 19.8 $\pm$ 6.7 & 0.10 & 5.25 & 2.5 $\pm$ 7.0 & 0.90 & 1.51 \\
008 pudding box & 10.9 $\pm$ 10.2 & 0.10 & 5.51 & 7.0 $\pm$ 9.1 & 0.30 & 9.38 & 7.3 $\pm$ 10.7 & 0.60 & 0.46 \\
\rowcolor{Gray}
009 gelatin box & 14.3 $\pm$ 9.2 & 0.10 & 3.49 & 13.0 $\pm$ 10.6 & 0.40 & 6.91 & 0.8 $\pm$ 1.6 & 0.80 & 1.83 \\
010 potted meat can* & 20.7 $\pm$ 2.8 & 0.00 & 4.74 & 21.0 $\pm$ 2.6 & 0.00 & 8.70 & 7.6 $\pm$ 10.4 & 0.40 & 0.60 \\
\rowcolor{Gray}
011 banana* & 6.1 $\pm$ 8.0 & 0.40 & 3.38 & 8.1 $\pm$ 8.9 & 0.50 & 3.16 & 4.8 $\pm$ 9.1 & 0.80 & 2.09 \\
019 pitcher base* & 7.1 $\pm$ 8.0 & 0.30 & 8.50 & 6.3 $\pm$ 8.1 & 0.40 & 0.00 & 12.3 $\pm$ 11.9 & 0.40 & 0.98 \\
\rowcolor{Gray}
021 bleach cleanser* & 0.5 $\pm$ 0.6 & 0.80 & 6.50 & 9.9 $\pm$ 9.1 & 0.30 & 7.75 & 0.2 $\pm$ 0.2 & 1.00 & 5.69 \\
024 bowl & 5.7 $\pm$ 8.3 & 0.70 & 4.51 & 2.5 $\pm$ 5.1 & 0.80 & 2.83 & 3.4 $\pm$ 7.0 & 0.80 & 2.18 \\
\rowcolor{Gray}
025 mug* & 8.2 $\pm$ 9.5 & 0.40 & 5.94 & 3.7 $\pm$ 6.3 & 0.60 & 2.41 & 0.1 $\pm$ 0.0 & 1.00 & 4.64 \\
035 power drill* & 12.1 $\pm$ 12.1 & 0.20 & 4.91 & 14.7 $\pm$ 12.0 & 0.30 & 5.91 & 10.2 $\pm$ 11.4 & 0.20 & 1.49 \\
\rowcolor{Gray}
036 wood block & 22.2 $\pm$ 4.2 & 0.00 & 6.65 & 24.0 $\pm$ 2.0 & 0.00 & 1.94 & 10.7 $\pm$ 12.4 & 0.50 & 1.84 \\
037 scissors* & 8.2 $\pm$ 8.5 & 0.30 & 2.94 & 5.1 $\pm$ 7.1 & 0.50 & 1.26 & 7.8 $\pm$ 11.3 & 0.60 & 1.74 \\
\rowcolor{Gray}
040 large marker & 10.1 $\pm$ 9.7 & 0.40 & 1.65 & 6.8 $\pm$ 9.9 & 0.60 & 4.01 & 7.3 $\pm$ 10.4 & 0.50 & 1.94 \\
052 extra large clamp & 3.6 $\pm$ 6.0 & 0.40 & 4.09 & 3.1 $\pm$ 6.1 & 0.60 & 7.46 & 5.1 $\pm$ 8.4 & 0.60 & 3.22 \\
\rowcolor{Gray}
061 foam brick & 21.3 $\pm$ 2.0 & 0.00 & 3.51 & 20.9 $\pm$ 1.3 & 0.00 & 7.81 & 0.1 $\pm$ 0.0 & 1.00 & 1.46 \\ \midrule
Average & 12.7 $\pm$ 6.5 & 0.24 & 4.94 & 12.4 $\pm$ 6.8 & 0.28 & 6.42 & 4.6 $\pm$ 6.7 & 0.73 & 2.81 \\ \bottomrule
    \end{tabular}}
\end{center}
\caption{Detailed results for the DexYCB and HO3D test set with grasp references from a static grasp synthesis method \cite{jiang2021graspTTA}. HO3D objects are marked by *.}
\label{tab:exp1_test_gtta_full}
\end{table*}

==> chapters/04_hoi_generation/dgrasp/sections/tables/table_gtta_train.tex <==
\begin{table*}[t]
\begin{center}
\resizebox{0.8\linewidth}{!}{
    \begin{tabular}{@{}l|c|c|c|c|c|c|c|c|c}
        \toprule
            \multicolumn{1}{c}{} & \multicolumn{3}{c|}{Jiang \textit{et. al} \cite{jiang2021graspTTA}+PD} & \multicolumn{3}{c|}{Jiang \textit{et. al} \cite{jiang2021graspTTA}+IK} & \multicolumn{3}{c}{Ours} \\ \midrule
        Object  & SimDist [mm/s] $\downarrow$ & Success $\uparrow$  & Interp. [$cm^3$]   & SimDist [mm/s] $\downarrow$ & Success $\uparrow$ & Interp. [$cm^3$] & SimDist [mm/s] $\downarrow$ & Success $\uparrow$ &  Interp. [$cm^3$]\\ \midrule
002 master chef can & 24.0 $\pm$ 1.5 & 0.00 & 6.39 & 24.0 $\pm$ 1.6 & 0.00 & 16.19 & 2.6 $\pm$ 7.5 & 0.90 & 2.70 \\
\rowcolor{Gray}
003 cracker box* & 22.8 $\pm$ 2.4 & 0.00 & 6.97 & 22.8 $\pm$ 2.5 & 0.00 & 8.18 & 6.0 $\pm$ 10.3 & 0.70 & 5.80 \\
004 sugar box* & 14.7 $\pm$ 8.5 & 0.10 & 5.60 & 15.2 $\pm$ 8.7 & 0.10 & 10.45 & 1.4 $\pm$ 5.3 & 0.95 & 4.03 \\
\rowcolor{Gray}
005 tomato soup can & 14.8 $\pm$ 9.1 & 0.10 & 5.62 & 14.6 $\pm$ 9.0 & 0.10 & 11.51 & 3.8 $\pm$ 8.7 & 0.85 & 5.76 \\
006 mustard bottle* & 5.6 $\pm$ 7.2 & 0.30 & 5.66 & 5.2 $\pm$ 7.3 & 0.50 & 10.61 & 0.8 $\pm$ 2.8 & 0.95 & 5.14 \\
\rowcolor{Gray}
007 tuna fish can & 20.9 $\pm$ 1.7 & 0.00 & 2.88 & 21.4 $\pm$ 1.7 & 0.00 & 4.84 & 0.3 $\pm$ 0.5 & 0.90 & 2.03 \\
008 pudding box & 11.0 $\pm$ 10.3 & 0.10 & 4.92 & 10.9 $\pm$ 10.2 & 0.10 & 7.88 & 6.2 $\pm$ 10.1 & 0.70 & 0.91 \\
\rowcolor{Gray}
009 gelatin box & 14.1 $\pm$ 8.7 & 0.10 & 3.89 & 14.3 $\pm$ 9.2 & 0.10 & 8.38 & 1.7 $\pm$ 5.9 & 0.90 & 1.44 \\
010 potted meat can* & 20.4 $\pm$ 2.9 & 0.00 & 3.96 & 20.7 $\pm$ 2.8 & 0.00 & 6.89 & 7.1 $\pm$ 11.0 & 0.65 & 0.46 \\
\rowcolor{Gray}
011 banana* & 4.4 $\pm$ 6.1 & 0.30 & 3.52 & 6.1 $\pm$ 8.0 & 0.40 & 2.33 & 7.0 $\pm$ 9.4 & 0.45 & 3.18 \\
019 pitcher base* & 6.4 $\pm$ 8.4 & 0.50 & 8.11 & 7.1 $\pm$ 8.0 & 0.30 & 13.64 & 6.4 $\pm$ 10.1 & 0.65 & 1.56 \\
\rowcolor{Gray}
021 bleach cleanser* & 0.8 $\pm$ 1.9 & 0.90 & 5.76 & 0.5 $\pm$ 0.6 & 0.80 & 6.82 & 2.1 $\pm$ 6.4 & 0.90 & 4.89 \\
024 bowl & 5.5 $\pm$ 8.0 & 0.70 & 4.93 & 5.7 $\pm$ 8.3 & 0.70 & 3.24 & 5.2 $\pm$ 7.7 & 0.40 & 1.78 \\
\rowcolor{Gray}
025 mug* & 7.9 $\pm$ 9.4 & 0.50 & 4.32 & 8.2 $\pm$ 9.5 & 0.40 & 2.19 & 1.3 $\pm$ 5.2 & 0.95 & 4.78 \\
035 power drill* & 12.3 $\pm$ 12.0 & 0.20 & 5.84 & 12.1 $\pm$ 12.1 & 0.20 & 8.40 & 11.4 $\pm$ 11.5 & 0.20 & 1.27 \\
\rowcolor{Gray}
036 wood block & 22.0 $\pm$ 4.6 & 0.00 & 7.28 & 22.2 $\pm$ 4.2 & 0.00 & 5.06 & 2.6 $\pm$ 7.5 & 0.90 & 2.99 \\
037 scissors* & 5.0 $\pm$ 7.5 & 0.30 & 2.37 & 8.2 $\pm$ 8.5 & 0.30 & 1.50 & 0.7 $\pm$ 1.4 & 0.85 & 2.18 \\
\rowcolor{Gray}
040 large marker & 10.3 $\pm$ 9.6 & 0.40 & 1.86 & 10.1 $\pm$ 9.7 & 0.40 & 3.41 & 7.2 $\pm$ 9.6 & 0.55 & 0.92 \\
052 extra large clamp & 3.6 $\pm$ 5.9 & 0.40 & 4.97 & 3.6 $\pm$ 6.0 & 0.40 & 8.21 & 3.4 $\pm$ 7.2 & 0.65 & 3.37 \\
\rowcolor{Gray}
061 foam brick & 20.9 $\pm$ 1.8 & 0.00 & 3.46 & 21.3 $\pm$ 2.0 & 0.00 & 6.56 & 1.3 $\pm$ 5.1 & 0.95 & 1.66 \\ \midrule
Average & 12.4 $\pm$ 6.4 & 0.25 & 4.92 & 12.7 $\pm$ 6.5 & 0.24 & 7.31 & 3.9 $\pm$ 7.2 & 0.75 & 2.84 \\ \bottomrule
    \end{tabular}}
\end{center}
\caption{Detailed results for the DexYCB and HO3D train set with grasp references from a static grasp synthesis method \cite{jiang2021graspTTA}. HO3D objects are marked by *.}
\label{tab:exp1_train_gtta_full}
\end{table*}

==> chapters/04_hoi_generation/dgrasp/sections/tables/table_motion.tex <==
\begin{table}[t]
	\centering
	\resizebox{0.8\columnwidth}{!}{%
		\begin{tabular}{ll|cc}
		
			\toprule

			& Models & MPE [mm] $\downarrow$ & Geodesic [rad.] $\downarrow$  \\
			
			\midrule

            & Flat-RL & 0.55 & 1.66 \\

            & \gc Ours+static grasp & \gc 0.45 & \gc 1.46 \\
            & Ours+learned policy & 0.30 & 0.92 \\

            & \gc \textbf{Ours} & \gc \textbf{0.08}  & \gc \textbf{0.52}  \\

			
			\bottomrule
		\end{tabular}%
	}

	\caption{\textbf{Evaluation of motion synthesis}. We compare our model with a standard RL baseline (Flat-RL) and different variants of our method. We observe that our hierarchical framework outperforms Flat-RL. Furthermore, an active grasping policy during motion synthesis is key to solving the task, as indicated by the performance drop for Ours+static grasp.}
	\label{tab:motion}
\end{table}{}



==> chapters/04_hoi_generation/dgrasp/sections/tables/table_rebuttal_generalization.tex <==
\newcommand{\greycellcol}{\cellcolor[HTML]{E4E4E4}}
\begin{table}[h!]
	\centering
	\resizebox{0.78\columnwidth}{!}{%
		\begin{tabular}{l|ll|ccc}
		
			\toprule

			& & Models & Success $\uparrow$ & SimDist [mm/s] $\downarrow$ & Interp. [$cm^3$] $\downarrow$  \\
			
			\midrule
			\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{UO}}}
			& \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{UO-1}}}
            & GT+PD & 0.41 & $10.7 \pm 9.9 $ & 0.24 \\
            & & \greycellcol \textbf{Ours} & \greycellcol \textbf{0.83}  & \greycellcol $\mathbf{3.3 \pm 7.7}$  & \greycellcol \textbf{0.0} \\

			\cmidrule{2-6}
			& \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{UO-2}}}
            & GT+PD & 0.3 & $15.5 \pm 10.4$ & 0.49 \\
            & & \greycellcol \textbf{Ours} & \greycellcol \textbf{0.59}  & \greycellcol $\mathbf{8.4 \pm 10.4}$  & \greycellcol \textbf{0.0} \\
			
			\midrule
			& \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{UG}}}
            & Ours PO & 0.42  & $12.4 \pm 10.4$  & 0.14 \\
%             % \rowcolor{Gray}
            & & \greycellcol \textbf{Ours AO} & \greycellcol \textbf{0.61} & \greycellcol $\mathbf{6.9 \pm 7.9}$ & \greycellcol \textbf{0.0}  \\
            % \rowcolor{Gray}

			\cmidrule{2-6}
			& \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{IB}}}
            % & Flat-RL & 0.55 & 1.66 \\
%             % \rowcolor{Gray}
%             & \greycellcol Ours+static grasp & \greycellcol 0.45 & \greycellcol 1.46 \\
            & CO [11] +PD & 0.6 & $6.5 \pm 5.8$ & 11. 7 \\
%             % \rowcolor{Gray}
            & & \greycellcol \textbf{Ours} & \greycellcol \textbf{0.81}  & \greycellcol $\mathbf{1.9 \pm 3.6}$ & \greycellcol \textbf{0.19}  \\
            % \rowcolor{Gray}
			
			\bottomrule
		\end{tabular}%
	}
    \vspace{-0.2cm}
	\caption{\footnotesize{Generalization to unseen object sets (UO), a policy trained over all objects evaluated on unseen grasp labels (UG), and a policy trained and evaluated on grasp labels from HO3D images (IB).}}
	\label{tab:unseen_obj}
\end{table}{}



==> chapters/05_handover/content/introduction.tex <==
\chapter{Introduction}
\label{ch:handover:introduction}

==> chapters/05_handover/handoversim2real/figures/fig_user_questionnaire.tex <==
\begin{figure*}[t!]
 % \vspace{-2mm}
 \centering
 \includegraphics[width=0.9\linewidth]{\dir/handoversim2real/figures/supp_user/rating_ours_1.pdf}
 \includegraphics[width=0.9\linewidth]{\dir/handoversim2real/figures/supp_user/rating_ours_2.pdf}
 % \vspace{-2mm}
 \caption{\small User's ranking with each statement for \textbf{our method} in the user evaluation. Each color denotes a different a degree of agreement. The length of the bar denotes the count of the users. For each bar, the center count of ``Neither agree or disagree'' is aligned with 0 in the horizontal axis. In the top figure, a higher agreement score (orange) indicates a better performance, while in the bottom figure, a lower agreement score (green) indicates a better performance.}
 % \vspace{-2mm}
 \label{fig:h2r:user_ours}
\end{figure*}

==> chapters/05_handover/handoversim2real/figures/real_world_limitation.tex <==
\begin{figure}[ht]
    \centering
    
    % First row of images
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{\dir/synh2r/sections/figures/seqs/synh2r_1.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{\dir/synh2r/sections/figures/seqs/synh2r_2.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{\dir/synh2r/sections/figures/seqs/synh2r_3.png}
    \end{subfigure}

    % Caption for the first row
    \caption{First set of images showing ...}
    
    \vspace{2em} % Space between rows

    % Second row of images
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{\dir/synh2r/sections/figures/seqs/handoversim2real_1.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{handoversim2real_2.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{handoversim2real_3.png}
    \end{subfigure}

    % Caption for the second row
    \caption{Second set of images showing ...}

\end{figure}

==> chapters/05_handover/handoversim2real/sections/00_abstract.tex <==
\begin{abstract}
\vspace{-2mm}
We propose the first framework to learn control policies for vision-based human-to-robot handovers, a critical task for human-robot interaction. While research in Embodied AI has made significant progress in training robot agents in simulated environments, interacting with humans remains challenging due to the difficulties of simulating humans. Fortunately, recent research has developed realistic simulated environments for human-to-robot handovers. Leveraging this result, we introduce a method that is trained with a human-in-the-loop via a two-stage teacher-student framework that uses motion and grasp planning, reinforcement learning, and self-supervision. We show significant performance gains over baselines on a simulation benchmark, sim-to-sim transfer and sim-to-real transfer. Video and code are available at \footnotesize{\url{https://handover-sim2real.github.io}}.
\end{abstract}
\vspace{-5mm}

==> chapters/05_handover/handoversim2real/sections/02_related_work.tex <==
\section{Related Work}

\paragraph{Human-to-Robot Handovers}
Encouraging progress in hand and object pose estimation~\cite{hasson:cvpr2019,liu:cvpr2021,li:cvpr2022} has been achieved, aided by the introduction of large hand-object interaction datasets~\cite{garcia-hernando:cvpr2018,hampali:cvpr2020,brahmbhatt:eccv2020,moon:eccv2020,taheri:eccv2020,chao:cvpr2021,ye:iccv2021,kwon:iccv2021,liu:cvpr2022, fan2023arctic}. These developments enable applying model-based grasp planning~\cite{bicchi:icra2000,miller:ram2004,bohg:tro2014}, a well-studied approach in which full pose estimation and tracking are needed, to H2R handovers~\cite{sanchez-matilla:ral2020,chao:cvpr2021}. However, these methods require the 3D shape models of the object and cannot handle unseen objects.
Alternatively, some recent works~\cite{rosenberger:ral2021,yang:icra2021,yang:icra2022,duan:tcds, marturi:2019dynamic} achieve H2R handover by employing learning-based grasp planners to generate grasps for novel objects from raw vision inputs such as images or point clouds~\cite{morrison:rss2018,mousavian:iccv2019}. 
While promising results have been shown, these methods work only on an open-loop sequential setting in which the human hand has to stay still once the robot starts to move~\cite{rosenberger:ral2021}, or need complex hand-designed cost functions for grasp selection~\cite{yang:icra2021} and robot motion planning~\cite{yang:icra2022, marturi:2019dynamic} for reactive handovers, which requires expertise in robot motion and control. 
Hence, these methods are difficult to reproduce and deploy to new environments.
Progress towards dynamic simultaneous motion has been shown by a learning-based method \cite{wang:corl2021a}, using state inputs, leaving an open challenge for training policies that receive visual input directly.
In contrast, we propose to learn control policies together with grasp prediction for handovers in an end-to-end manner from segmented point clouds with a deep neural net. 
To facilitate easy and fair comparisons among different handover methods, \cite{chao:icra2022} propose a physics-simulated environment with diverse objects and realistic human handover behavior collected by a mocap system~\cite{chao:cvpr2021}. They provide benchmark results of several previous handover systems, including a learning-based grasping policy trained with static objects~\cite{wang:corl2021b}. 
However, learning a safe and efficient handover policy is not trivial with a human-in-the-loop, which we address in this work.
\vspace{-3mm}
\paragraph{Policy Learning for Grasping}
Object grasping is an essential skill for many robot tasks, including handovers. 
Prior works usually generate grasp poses given a known 3D object geometry such as object shape or pose~\cite{bicchi:icra2000,miller:ram2004,bohg:tro2014}, which is nontrivial to obtain from real-world sensory input such as images or point clouds. 
To overcome this, recent works train deep neural networks to predict grasps from sensor data~\cite{kleeberger2020survey} and compute trajectories to reach the predicted grasp pose. 
Though 3D object geometry is no longer needed, the feasibility is not guaranteed since the grasp prediction and trajectory planning are computed separately. 
Some recent works directly learn grasping policies given raw sensor data. 
\cite{kalashnikov:corl2018} propose a self-supervised RL framework based on RGB images to learn a deep Q-function from real-world grasps. 
To improve data efficiency, \cite{song:ral2020} use a low-cost handheld device to collect grasping demonstrations with a wrist-mounted camera. They train an RL-based 6-DoF closed-loop grasping policy with these demonstrations.
\cite{wang:corl2021b} combines imitation learning from expert data with RL to learn a control policy for object grasping from point clouds. 

Although this method performs well in HandoverSim \cite{chao:icra2022} when the human hand is not moving, it has difficulty coordinating with a dynamic human hand since the policy is learned with static objects. 
Instead, our policy is directly learned from large-scale dynamic hand-object trajectories obtained from the real world.
To facilitate the training for the dynamic case, we propose a two-stage teacher-student framework, that is conceptually inspired by \cite{chen:corl2021}, which has been proven critical through experiments.


==> chapters/05_handover/handoversim2real/tables/table_main_exp_pruned.tex <==
\begin{table}[t]
 % \vspace{-2mm}
 \centering
 \small
 % \setlength{\tabcolsep}{6pt}
 \begin{tabular}{l|l|cccc}

  \hline
  & & \multirow{2}{*}{success (\%)} & \multicolumn{3}{c}{failure (\%)} \\
  & & & contact & drop & timeout \\
  \hline
  \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{Sequential}}}
  & OMG Planner \cite{wang2020manipulation} $\dagger$        & 62.50 &  27.78          & ~~8.33 & ~~1.39 \\
  & \gc Yang et al. \cite{yang2021reactive} $\dagger$  & \gc 64.58  &  \gc 17.36          &  \gc 11.81          & \gc ~~6.25        \\  
\cline{2-6}
  & GA-DDPG \cite{wang2021goal}   & 50.00         & ~\textbf{4.86} &  19.44          &  25.69      \\
  & \gc GA-DDPG \cite{wang2021goal} finetuned  & \gc 57.18        & \gc ~6.48 &  \gc 27.08          &  \gc ~9.26 \\
 
  & Ours    & \textbf{75.23} & ~9.26 & \textbf{13.43} & ~\textbf{2.08}   \\
%   & \gc Ours + grasp pred. & \gc 71.07 & \gc 5.43 & \gc tbd & \gc tbd  & \gc ~6.00 & \gc 16.20 & \gc ~6.73 \\ 
%   Ours (hand avg + pred)  w/o hold & 43.73 & tbd & tbd & tbd  & 16.3 & ~21.5 & ~18.40 \\ 
\hline

  \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Simult.}}}
  
  & GA-DDPG \cite{wang2021goal} &  36.81         &  ~9.03          &  25.00          &  29.17   \\
  & \gc GA-DDPG \cite{wang2021goal} finetuned  & \gc 54.86         & \gc ~\textbf{6.71} &  \gc 26.39          & \gc 12.04        \\
 
  & Ours   & \textbf{68.75} & ~8.80 & \textbf{17.82} & ~\textbf{4.63}      \\
%   & \gc Ours + grasp pred & \gc 70.37 & \gc 4.860 & \gc tbd & \gc tbd  & \gc 7.64 & \gc ~14.71 & \gc ~6.95 \\ 
  
\bottomrule
  
 \end{tabular}

 \caption{\textbf{HandoverSim Benchmark Evaluation.} Comparison of our method against various baselines from the HandoverSim benchmark \cite{chao2022handoversim}. In the sequential setting, we find that our baseline achieves better overall success rates than the baselines. In the simultaneous setting, we outperform the applicable baselines by large margins. The results for our method are averaged across 3 random seeds. $\dagger$: both methods \cite{wang2020manipulation,yang2021reactive} are evaluated with ground-truth states in \cite{chao2022handoversim} and thus are not directly comparable with ours.}

 \label{tab:h2r:quantitative}
\end{table}

==> chapters/05_handover/handoversim2real/tables/table_pilot_detailed.tex <==
\begin{table*}[t!]
 % \vspace{-2mm}
 \centering
 \footnotesize
 \setlength{\tabcolsep}{1.8pt}
 \begin{tabular}{l||C{0.78cm}C{0.78cm}|C{0.78cm}C{0.78cm}|C{0.78cm}C{0.78cm}|C{0.78cm}C{0.78cm}||C{0.78cm}C{0.78cm}|C{0.78cm}C{0.78cm}|C{0.78cm}C{0.78cm}|C{0.78cm}C{0.78cm}}
                           & \multicolumn{16}{c}{subject 2: overall}                                                                                                                                                                                                                           \\
                           & \multicolumn{8}{c||}{GA-DDPG~\cite{wang:corl2021b}}                                                                             & \multicolumn{8}{c}{Ours}                                                                                                        \\
                           & \multicolumn{2}{c|}{pose 1} & \multicolumn{2}{c|}{pose 2} & \multicolumn{2}{c|}{pose 3} & \multicolumn{2}{c||}{mean}            & \multicolumn{2}{c|}{pose 1} & \multicolumn{2}{c|}{pose 2} & \multicolumn{2}{c|}{pose 3} & \multicolumn{2}{c}{mean}              \\
                           & succ.       & time          & succ.       & time          & succ.       & time          & succ.              & time             & succ.       & time          & succ.       & time          & succ.       & time          & succ.              & time             \\
  \hline
  011\_banana              & ~~2 / ~~2   & 11.154        & ~~2 / ~~2   & 12.372        & ~~2 / ~~2   & ~~8.951       & \textbf{~~6 / ~~6} & 10.826           & ~~2 / ~~2   & 10.546        & ~~1 / ~~2   & 10.408        & ~~2 / ~~2   & ~~8.006       & ~~5 / ~~6          & \textbf{~~9.510} \\
  037\_scissors            & ~~2 / ~~2   & 10.229        & ~~0 / ~~2   & --            & ~~1 / ~~2   & ~~9.243       & ~~3 / ~~6          & 10.076           & ~~2 / ~~2   & ~~8.465       & ~~1 / ~~2   & ~~9.638       & ~~2 / ~~2   & ~~8.477       & \textbf{~~5 / ~~6} & \textbf{~~8.891} \\
  006\_mustard\_bottle     & ~~1 / ~~2   & ~~9.476       & ~~0 / ~~2   & --            & ~~1 / ~~2   & 10.479        & ~~2 / ~~6          & 10.201           & ~~2 / ~~2   & ~~8.433       & ~~0 / ~~2   & --            & ~~2 / ~~2   & ~~9.445       & \textbf{~~4 / ~~6} & \textbf{~~8.939} \\
  024\_bowl                & ~~1 / ~~2   & 11.101        & ~~0 / ~~2   & --            & ~~2 / ~~2   & ~~9.149       & \textbf{~~3 / ~~6} & \textbf{~~9.161} & ~~0 / ~~2   & --            & ~~1 / ~~2   & ~~9.720       & ~~2 / ~~2   & 13.692        & \textbf{~~3 / ~~6} & 12.447           \\
  040\_large\_marker       & ~~2 / ~~2   & 10.707        & ~~0 / ~~2   & --            & ~~2 / ~~2   & ~~9.314       & ~~4 / ~~6          & \textbf{10.010}  & ~~2 / ~~2   & ~~9.419       & ~~1 / ~~2   & 15.882        & ~~2 / ~~2   & 13.537        & \textbf{~~5 / ~~6} & 12.041           \\
  003\_cracker\_box        & ~~0 / ~~2   & --            & ~~0 / ~~2   & --            & ~~0 / ~~2   & --            & ~~0 / ~~6          & --               & ~~1 / ~~2   & 11.925        & ~~0 / ~~2   & --            & ~~1 / ~~2   & 12.989        & \textbf{~~2 / ~~6} & 11.596           \\
  052\_extra\_large\_clamp & ~~2 / ~~2   & 14.533        & ~~1 / ~~2   & ~~9.562       & ~~2 / ~~2   & ~~9.680       & \textbf{~~5 / ~~6} & \textbf{11.599}  & ~~2 / ~~2   & 14.521        & ~~2 / ~~2   & 13.460        & ~~1 / ~~2   & 36.778        & \textbf{~~5 / ~~6} & 13.103           \\
  008\_pudding\_box        & ~~2 / ~~2   & 10.098        & ~~0 / ~~2   & --            & ~~2 / ~~2   & ~~9.037       & \textbf{~~4 / ~~6} & ~~9.567          & ~~2 / ~~2   & ~~8.668       & ~~0 / ~~2   & --            & ~~2 / ~~2   & ~~9.825       & \textbf{~~4 / ~~6} & \textbf{~~9.247} \\
  010\_potted\_meat\_can   & ~~1 / ~~2   & ~~9.919       & ~~0 / ~~2   & --            & ~~2 / ~~2   & 11.063        & ~~3 / ~~6          & 10.493           & ~~2 / ~~2   & ~~8.442       & ~~0 / ~~2   & --            & ~~2 / ~~2   & ~~8.943       & \textbf{~~4 / ~~6} & \textbf{~~8.693} \\
  021\_bleach\_cleanser    & ~~2 / ~~2   & 10.355        & ~~1 / ~~2   & 12.233        & ~~0 / ~~2   & --            & ~~3 / ~~6          & 10.311           & ~~2 / ~~2   & ~~8.771       & ~~0 / ~~2   & --            & ~~2 / ~~2   & 10.997        & \textbf{~~4 / ~~6} & \textbf{~~9.884} \\
  \hline
  total                    & 15 / 20     & 10.784        & ~~4 / 20    & 11.134        & 14 / 20     & ~~9.678       & 33 / 60            & \textbf{10.357}  & 17 / 20     & ~~9.774       & ~~6 / 20    & 12.031        & 18 / 20     & 10.387        & \textbf{41 / 60}   & 10.373           \\
 \end{tabular} 
 % \vspace{-2mm}
 \caption{\small The pilot study results of \textbf{subject 2}. We present the results separately for the right-hand handovers (top), the left-hand handovers (middle), and overall (bottom). We report both the success rate (``succ.'') and the completion time (``time''). Our method outperforms GA-DDPG~\cite{wang:corl2021b} in the success rate.}
 % \vspace{-2mm}
 \label{tab:h2r:pilot_subject_2}
\end{table*}

==> chapters/05_handover/handoversim2real/tables/table_rebuttal.tex <==
\begin{table}[t]
 \centering
 \small
 % \setlength{\tabcolsep}{6pt}
  \resizebox{0.75\columnwidth}{!}{%
 \begin{tabular}{l|cccc}

  \multirow{2}{*}{HandoverSim benchmark} & \multirow{2}{*}{success (\%)} &  \multicolumn{3}{c}{failure (\%)} \\
  & & contact & drop & timeout \\
  \hline

   w/ RGBDM + ResNet18 & 34.10  & ~~\textbf{6.20} &  45.80     &  13.90          \\
  \rowcolor{Gray}
   w/ Kinect noise & 59.49 & 13.19 &  19.68 &  ~~7.64         \\ 


   w/ third person view & 60.42  & ~~9,95 &  25.69     &  ~~3.94          \\
     \rowcolor{Gray}
   w/o aux prediction & 70.60  & 10.65 &  16.20     & ~~2.54          \\

 

  \textbf{Ours} & \textbf{75.23} & ~~9.26 & \textbf{13.43} & ~~\textbf{2.08} \\ \hline

 \end{tabular}
 }
 \caption{\textbf{Ablation.} We ablate the our method's vision components and the auxiliary loss. Results are averaged over 3 random seeds.
%  \wei{Refer ``RGBDM" in the main text?}
 }
 \label{tab:h2r:ebuttal}
\end{table}

==> chapters/05_handover/handoversim2real/tables/table_sim2sim.tex <==
\begin{table*}[t]
 % \vspace{-2mm}
 \centering
 \small
 % \setlength{\tabcolsep}{6pt}
 \begin{tabular}{l|l|cccc|cccc}
  \hline
  \multicolumn{9}{c}{Sim-to-Sim} \\
  \hline
  & & \multirow{2}{*}{success (\%)} & \multicolumn{3}{c|}{mean accum time (s)} & \multicolumn{4}{c}{failure (\%)} \\
  & & & exec & plan & total & contact & drop & timeout & total \\
  \hline
  \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Sequential}}}
%   & OMG Planner~\cite{wang:rss2020}        & 58.33 & 8.304          & ~~2.486          &  10.790          &  32.64          & ~~\textbf{7.64} & ~\textbf{1.39} \\
%   & \gc Yang et al.~\cite{yang:icra2021} & \gc 56.25  & \gc \textbf{4.414}  & \gc ~~0.617          & \gc 5.031          &  \gc 16.67          &  \gc 18.06          & \gc ~~9.03          \\
  & GA-DDPG~\cite{wang:corl2021b} &  19.44          & ~7.171          & ~0.175          & ~7.346          & \textbf{4.86} & 47.22          & 28.47   &   80.56    \\
  & \gc GA-DDPG~\cite{wang:corl2021b} finetuned  & \gc tbd         & \gc tbd        & \gc tbd & \gc tbd      & \gc tbd &  \gc tbd          &  \gc tbd    & \gc tbd    \\
  
  &  \textbf{Ours} & 44.21 & 7.666 & 0.236 & 7.901  & 9.49 & 40.51 & 5.79 & 55.79  \\ 
  
  & \gc \textbf{Ours w/o grasp  pred.} & \gc \textbf{54.40} & \gc 9.165 & \gc 0.239 & \gc 9.403  & \gc 7.87 & \gc \textbf{33.34} & \gc \textbf{4.40} & \gc \textbf{45.60} \\
%   Ours (hand avg + pred)  w/o hold & 43.73 & tbd & tbd & tbd  & 16.3 & ~21.5 & ~18.40 \\ 
 

  \hline

  \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Simult.}}}
  
  & GA-DDPG~\cite{wang:corl2021b} & 11.11          & \textbf{4.678} & ~\textbf{0.168}          & ~\textbf{4.847} & 15.97          & 48.61          & 24.31  & 88.89        \\
  & \gc GA-DDPG~\cite{wang:corl2021b} finetuned  & \gc tbd          & \gc tbd          & \gc tbd & \gc tbd         & \gc tbd &  \gc tbd          & \gc tbd & \gc tbd      \\
 
  & \textbf{Ours}    & 39.58 & 6.129 & 0.220 & 6.349  & 9.03 & 43.75  & 7.64 & 60.42   \\
  & \gc \textbf{Ours w/o grasp pred.} & \gc \textbf{47.92} & \gc 7.610 & \gc 0.222 & \gc 7.833  & \gc \textbf{10.65} & \gc \textbf{35.88} & \gc \textbf{5.56}  & \gc \textbf{52.08} \\ 
  
\bottomrule
  
 \end{tabular}
 % \vspace{-2mm}
 \caption{\textbf{Sim-to-Sim experiment}. We evaluate sim-to-sim transfer of the learning-based methods, i.e., we train policies in Pybullet \cite{kalevatykh:2020} and evaluate them in Isaac Gym\cite{makoviychuk:neuripstdb2021}. We find that our method has much better transfer capabilities than GA-DDPG \cite{wang:corl2021b}, in both the sequential and the simultaneous setting. Closer analysis indicates that part of the performance drop of our method is caused by the grasp prediction policy not transferring well, which we see when comparing 'Ours' against 'Ours w/o grasp pred.'. Results are averaged across 3 random seeds.}
 % \vspace{-2mm}
 \label{tab:h2r:sim2sim}
\end{table*}

==> chapters/05_handover/synh2r/sections/00_abstract.tex <==
\begin{abstract}

Vision-based human-to-robot handover is an important and challenging task in human-robot interaction. Recent work has attempted to train robot policies by interacting with dynamic virtual humans in simulated environments, where the policies can later be transferred to the real world. However, a major bottleneck is the reliance on human motion capture data, which is expensive to acquire and difficult to scale to arbitrary objects and human grasping motions. In this paper, we introduce a framework that can generate plausible human grasping motions suitable for training the robot. To achieve this, we propose a hand-object synthesis method that is designed to generate handover-friendly motions similar to humans. This allows us to generate synthetic training and testing data with 100x more objects than previous work. In our experiments, we show that our method trained purely with synthetic data is competitive with state-of-the-art methods that rely on real human motion data both in simulation and on a real system. In addition, we can perform evaluations on a larger scale compared to prior work. With our newly introduced test set, we show that our model can better scale to a large variety of unseen objects and human motions compared to the baselines. 

\end{abstract}



==> chapters/05_handover/synh2r/sections/01_introduction.tex <==
\input{\dir/synh2r/sections/figures/fig_teaser}
\section{Introduction}

In the previous chapter, we presented a framework to perform human-to-robot handovers, a crucial task in human-robot interaction (HRI)~\cite{ortenzi2021object}. Seamless human-to-robot handovers will enable robots to assist humans in many domains, such as manufacturing settings, elderly homes, or rehabilitation. In unknown scenarios, robots will encounter objects and human behavior that they have not previously experienced. Therefore, robots should be flexible in handling unseen objects and human behavior.

Collecting training experiences for robots in the real world is prohibitively inefficient and unsafe for humans. Therefore, our work on H2R handovers~\cite{chao2022handoversim,christen:2023:handoversim2real} has trained robot policies in simulation by allowing the robot to interact with a simulated human partner, and later transfer the trained policies onto real-world platforms. While this improves the scalability of collecting training experiences for the robot, the pipeline for simulating the human counterpart remains challenging to scale. In order to simulate realistic human motions for handovers, prior work~\cite{chao2022handoversim,christen:2023:handoversim2real,pang2021towards, christen:2019:drlhs} relies on motion capture data of hand-object interactions~\cite{chao2021dexycb}. The simulated environment for training robots is thus bounded by the object instances and human motions pre-captured in the mocap dataset. To train on novel objects or human motions, a tedious re-capturing of data with a mocap setup is required. This begs the question: can we automatically synthesize human handover motions on arbitrary objects for robot handover training, and thereby fully leverage the blessing of scalability from training in simulation?


Fortunately, our work in hand-object interaction synthesis (Part \ref{part:hoi}) holds the promise to generate natural and physically plausible human grasping motions, which can potentially alleviate the need for expensive motion capture. For example, D-Grasp (Chapter \ref{ch:hoi_generation:dgrasp}) generates hand motions that grasp an object and move it to a target pose using a reinforcement learning (RL) based policy. Despite their promise, these methods are still not readily applicable for human-to-robot handovers. For example, D-Grasp assumes a grasp pose reference as input and does not account for the handover-friendliness of such a grasp. For successful handovers, it is crucial to control the direction of approaching and the amount of free area for the robot to grasp the object. 

In this chapter, we combine human-to-robot handover training with hand-object motion synthesis (see \figref{fig:synh2r:teaser}). We build upon D-Grasp and propose a method that can generate natural human grasping motions that are suited for training robots without requiring any high-quality motion capture data. The first question is how to generate grasp references. Current static grasp generation pipelines do not offer controllability with respect to the grasp direction. This makes them unsuitable for handover since humans tend to hand over objects in a direction toward the robot and leave free space on the opposite side for the robot to grasp the object. Besides, we empirically discovered that off-the-shelf learning-based grasp generation models often struggle to generalize to objects beyond the training distribution. This limits their use on arbitrary object datasets without additional training. To this end, we propose an optimization-based grasp generation method that is conditioned on the approaching direction and incentivizes a stable human hand grasp that does not enclose an object fully. Since our grasp generation pipeline is non-learning based, it also does not suffer from generalization issues on unseen objects. We then generate hand pose references on a large set of objects, and pass them to D-Grasp to generate human grasping and handover motions. To improve the grasping of unseen objects, we also augment D-Grasp to condition on an object shape representation. With this pipeline, our method can synthesize diverse human motions for grasping unseen objects at a larger scale. This in turn allows us to leverage much more diverse human motions and objects in simulation to train the robot.


% Experiments
In our experiments, we first evaluate our approach on the HandoverSim benchmark \cite{chao2022handoversim}. We demonstrate that training our method from purely synthetic human motion data can achieve on-par performance with recent work that relies on high-quality motion capture data and uses the test objects during training. Furthermore, we introduce a new synthetic test set of 1174 unseen objects which exceeds the scale of previous benchmarks by 100x (see \tabref{tab:synh2r:related}). Our method outperforms the state-of-the-art baselines on this more challenging testbed. Lastly, we show that users do not recognize any significant differences between a policy trained on purely synthetic data versus a policy trained on real motion capture data, indicating the naturalness and plausibility of our generated human motions. This is an important insight that has implications for the training of robotic agents with simulated humans in the future.

In summary, we contribute:
\begin{itemize}
    \item A method to synthesize natural human handover motions that generalizes to unseen objects and integration of such motions into our human-to-robot handover training framework.
    \item A new synthetic test set that allows the evaluation of human-to-robot handovers on more than 1,000 unknown objects. 
    \item Experiments in simulation and on a real system showing our method performs on par with baselines that use high-quality motion capture data for training.
\end{itemize}


==> chapters/05_handover/synh2r/sections/02_related_work.tex <==
\section{Related Work}
\subsection{Grasp Synthesis for Dexterous Hands}

The problem of dexterous grasp synthesis involves determining optimal grasping poses given an object's mesh or point cloud and is generally categorized into two techniques: \textit{non-learning-based} and \textit{learning-based}. 

\textit{Learning-based} methods employ neural networks to predict grasps, leveraging motion capture grasp datasets~\cite{Jiang2021HandObjectCC,Karunratanakul2020GraspingFL,taheri:eccv2020} or synthetic datasets generated by their non-learning-based counterparts \cite{Miller2004GraspitAV,hasson:cvpr2019}. These methods predominantly rely on conditional variational autoencoder architectures, where the resulting grasps are stochastically sampled from latent space. To generalize to unseen shapes, the objects need to be close enough to the training distribution. In our approach, we use a non-learning based solution and hence do not suffer from generalization issues. \textit{Non-learning-based} methods have been employed to generate extensive synthetic datasets~\cite{Miller2004GraspitAV,Wang2022DexGraspNetAL,turpin2022grasp,turpin2023fast,hasson19obman}. \cite{Miller2004GraspitAV} employs collision detection algorithms to formulate stable grasps. In a different vein, some approaches employ differentiable force closure estimation~\cite{Wang2022DexGraspNetAL, Liu2021SynthesizingDA} for grasp generation. Works such as \cite{turpin2022grasp,turpin2023fast} exploit a differentiable simulation to synthesize grasps. In contrast to these works, our method can be conditioned on the grasp direction and does not rely on any simulator or force closure estimation.
Beyond static grasp synthesis, there are works~\cite{christen2022dgrasp,zhou2022toch,Xu2023UniDexGraspUR,Wu2022LearningGD,braun2023physically, zhang2024artigrasp} that focus on the temporal aspect of hand-object synthesis. D-Grasp \cite{christen2022dgrasp} introduces dynamic grasp synthesis to model hand-object interaction sequences, while \cite{Xu2023UniDexGraspUR} proposes a universal grasp policy generalizable to diverse objects. These methods utilize grasp reference poses to guide their RL-based policies. In our work, we present an RL policy that can be trained on a small set of YCB objects and generalize to unseen objects at inference time. We achieve this by combining grasp references from our non-learning based grasp optimization with an RL-based policy. 

\input{sections/tables/table_related}
\input{sections/figures/fig_method}


\subsection{Human-to-Robot Handovers}
Recent advances in human-to-robot (H2R) handover systems \cite{chao:icra2022, christen2023handover, pang:roman2021, sanchez-matilla:ral2020, rosenberger:ral2021, yang:icra2021, yang:icra2022, duan:tcds} show the potential of creating robust human-to-robot interaction frameworks. This progress has been driven by the surge of hand-object interaction datasets \cite{chao:cvpr2021, taheri:eccv2020, liu:cvpr2022, garcia-hernando:cvpr2018,hampali:cvpr2020,brahmbhatt:eccv2020,moon:eccv2020,ye:iccv2021,fan2023arctic}, which allows studying H2R handovers as a grasp planning problem \cite{Miller2004GraspitAV, bicchi:icra2000, bohg:tro2014}. These approaches require the exact knowledge of the 3D object shape, and hence do not generalize to unseen objects. To mitigate this, recent works leverage learning-based grasp predictions from vision input ~\cite{rosenberger:ral2021, yang:icra2021,yang:icra2022,duan:tcds, marturi:2019dynamic}. Rosenberger \etal~\cite{rosenberger:ral2021} use hand and object tracking and a grasp selection network to plan H2R handovers, which are executed in open-loop fashion. Yang \etal~\cite{yang:icra2021} propose a reactive H2R system that can generalize to unseen objects by selecting temporally consistent 6DoF grasps from GraspNet \cite{mousavian:iccv2019}. In \cite{yang:icra2022}, this work is improved by employing an MPC-based algorithm that adds reachability criteria to the motion planning. However, these methods either require the human hand to be stationary, complex hand-designed cost functions, and expertise in robot motion planning.  Chao \etal~\cite{chao:icra2022} introduce HandoverSim, a benchmark to evaluate handover policies in simulation. GA-DDPG \cite{wang:corl2021b} propose a vision-based method for grasping static objects, which can be deployed for H2R handovers. However, their method has difficulties in dynamic scenes with humans. Closest to our work, Christen \etal~\cite{christen2023handover} propose a framework to learn vision-based handover policies by training with human grasping motions from the DexYCB dataset \cite{chao:cvpr2021}. In contrast, our work uses synthetic handover motions generated by our method. Therefore, it does not require any real-world mocap data and allows scaling to a much more diverse set of training objects and motions.   




==> chapters/05_handover/synh2r/sections/04_method.tex <==
\input{\dir/synh2r/sections/figures/fig_method}
\section{Overview}
The goal of this chapter is to teach a robot agent to perform human-to-robot handovers by training purely on synthetic human motion data. The simulation setting follows HandoverSim \cite{chao2022handoversim} and consists of a tabletop scene with different objects, a robot, and a simulated human hand, as also described in Section \ref{sec:h2r:handoversim}. The robot comprises a 7-DoF Panda arm with a two-fingered gripper and a wrist-mounted RGB-D camera. The simulated hand replays human handover motions (either from motion capture or synthetic). The goal of the robot is to grasp the object from the human, without collision or dropping, and move it to a designated goal location.
Our framework comprises two stages, as shown in \figref{fig:synh2r:method_overview}. In the handover motion generation stage (left), we generate synthetic human-object interaction data over a large set of different objects. In the human-to-robot handover training stage, we leverage the synthetic data to train a vision-based human-to-robot handover policy in simulation, which can be transferred to a real system. 


\section{Synthetic Handover Motion Generation}
To synthesize human handover motions (\figref{fig:synh2r:method_overview} left), we first generate handover-friendly static grasp poses and then utilize these grasps as references to guide an RL-based policy inspired by D-Grasp \cite{christen:2022:dgrasp} to generate handover motions. 

\subsection{Grasp Reference Generation}
\label{sec:static_grasp_gen}
Our controllable grasp optimizer takes as input an object mesh $\pcvec_o$, a unified human hand mesh $\pcvec_h$ given by the parametric MANO hand model \cite{romero2017embodied}, and a grasp direction $\mathbf{v}_{\text{grasp}}$ defined by a three-dimensional vector pointing from the wrist joint to the object center. The MANO hand model \cite{romero2017embodied} is parameterized by a set of pose parameters $\textbf{q} \in \mathbb{R}^{45}$ and global hand pose $\posesix \in \mathbb{R}^{6}$ that includes 3D wrist translation and 3D wrist orientation. The pose parameters comprise 15 joints with 3DoF each. We use the lower dimensional Principal Component Analysis (PCA) space with 15 components to represent the pose parameters. As shown in \figref{fig:synh2r:method_overview} (left), we introduce a controllable grasp optimizer that outputs two keyframe hand poses—a \textit{pre-grasp pose} $\boldsymbol{\Phi}_{\text{pre}} = [\posesix_{\text{pre}}, \textbf{q}_{\text{pre}}]$ and a \textit{grasp reference pose} $\boldsymbol{\Phi}_{\text{grasp}} = [\posesix_{\text{grasp}}, \textbf{q}_{\text{grasp}}]$.
We first generate the pre-grasp pose, which is crucial to achieving stable grasping \cite{dasari2023learning}, and then optimize the grasp reference pose based on it. Both the pre-grasp pose and the grasp reference pose should adhere to the grasp direction $\mathbf{v}_{\text{grasp}}$. \\

\input{\dir/synh2r/sections/figures/fig_gripper}

\paragraph{Pre-Grasp Pose} $\boldsymbol{\Phi}_{\text{pre}}.$ We separately optimize the 6D global pre-grasp pose $\posesix_\text{pre}$, which includes the global wrist translation and wrist orientation, and the local finger pre-grasp pose $\textbf{q}_{\text{pre}}$. As shown in \figref{fig:synh2r:gripper}, we define the line connecting the middle fingertip to the thumb tip as the \textit{grasp axis}. Similarly, the vector originating from the wrist joint and pointing towards the midpoint of this connecting line is termed the hand's \textit{heading}. \\

\noindent\textbf{Gripper-like Finger Pose $\textbf{q}_{\text{pre}}$}. A two-fingered gripper typically has two adjustable fingers designed to grasp an object firmly from both sides. As illustrated in \figref{fig:synh2r:gripper}, this characteristic is emulated by considering the thumb as one finger of the gripper and grouping the other fingers as the second finger. The gripper-like finger pose $\textbf{q}_{\text{pre}}$ is derived by maximizing the separation between the thumb tip and the palm plane, i.e., the grasp axis. Specifically, the MANO hand is initialized in the flat hand pose $\textbf{q}_{\text{flat}}$ without any rotation or translation. By default, the flat hand is positioned in the xz-plane, with the palm oriented in the -y direction. The y-coordinate of the thumb tip, $\mathbf{x}^y_{\text{thumb}} (\textbf{q})$, is minimized to maximize its separation from the other fingers, resulting in gripper-like finger poses:
\begin{equation}
\textbf{q}_{\text{pre}} = \mathop{\argmin}\limits_{\textbf{q}}  
\mathbf{x}^y_{\text{thumb}}(\textbf{q};\textbf{q}_{\text{flat}}).
\end{equation}

\noindent We use the Adam optimizer~\cite{kingma2015adam} with a learning rate set at 0.003 for 300 iterations. Since we optimize in PCA space, the remaining four fingers converge to a natural pose, even though the objective focuses on the thumb's position. \\


\noindent\textbf{6D Global Pre-Grasp Pose $\posesix_\text{pre}$.} We visualize the process of determining the global 6D wrist pre-grasp pose in \figref{fig:synh2r:gripper}. We begin by sampling 3,000 points from the object mesh and identify the sampled point furthest from the object center along the grasp direction. The pre-grasp translation is computed as the distance between the object center and the furthest point with an added offset, ensuring there is no collision with the object. To get the pre-grasp global orientation, we first align the hand's heading with the grasp direction $\mathbf{v}_\text{grasp}$ (cf. \figref{fig:synh2r:gripper}). We then rotate the hand to grasp the slimmest part of the object. To this end, we project the object points onto a 2D plane orthogonal to the given grasp direction. We run PCA analysis on the projected 2D point set, which yields two principal components. We choose the component with the lower variance that corresponds to the object's narrowest width. Subsequently, the hand is rotated such that the grasp axis aligns with this narrowest segment.



\paragraph{Grasp Reference Pose} $\boldsymbol{\Phi}_{\text{grasp}}.$
The second part of our optimization generates a grasp reference pose. It takes as input the hand mesh $\pcvec_h$, the object mesh $\pcvec_o$, and the grasp direction $\mathbf{v}_{\text{grasp}}$. We initialize the hand in the pre-grasp pose $\boldsymbol{\Phi}_{\text{pre}}$ from the previous stage. Then, multiple losses are optimized to determine the grasp reference pose $\boldsymbol{\Phi}_{\text{grasp}}$:
\begin{equation}
\begin{aligned}
\boldsymbol{\Phi}_{\text{grasp}} &= \mathop{\argmin}\limits_{\boldsymbol{\Phi}} \mathcal{L}(\mathbf{{\pcvec}_h{(\boldsymbol{\Phi};\boldsymbol{\Phi_\text{pre}})}},\pcvec_o, \mathbf{v}_{\text{grasp}}),\\
\mathcal{L} &= \alpha \mathcal{L}_{\text{DP}} + \beta \mathcal{L}_{\text{C}} + \gamma \mathcal{L}_{\text{DF}} +  \delta \mathcal{L}_{\text{Ctrl}}.
\end{aligned}
\end{equation}
In the following computations, the object and hand vertices are sampled from the mesh surfaces only. The loss function $\mathcal{L}$ comprises the following components: \\

\noindent\textbf{Dual Penetration Loss $\mathcal{L}_{\text{DP}}$}. We employ a hand-centric penetration loss to minimize penetration during the optimization, similar to \cite{jiang2021hand}. We identifiy the object vertices that are situated inside the hand mesh and compute the penetration loss as the sum of the distances between these vertices and their nearest hand surface vertices:
\begin{equation}
    \begin{aligned}
            \mathcal{L}_{\text{DP}} = \sum_i \mathcal{L}^2(\mathbf{o}_i^{\text{in}}, \mathbf{h}^{\text{closest}}_i) +  \sum_j \mathcal{L}^2(\mathbf{h}_j^{\text{in}}, \mathbf{o}^{\text{closest}}_j),
    \end{aligned}
    \label{eq:dp_loss}
\end{equation}
where $\mathbf{o}_i^{\text{in}} \in \pcvec_o$ is the $i$-{th} object point inside the hand mesh and $\mathbf{h}^{\text{closest}}_i \in \pcvec_h$ is its closest vertex on the hand surface. While the hand-centric loss mitigates penetration by urging the object vertices toward their closest hand vertices, it is insufficient when entire fingertips are immersed within the object. To address this limitation, we additionally introduce an object-centric penetration loss, implemented in a symmetric manner (second term in \eqref{eq:dp_loss}).\\

\noindent\textbf{Contact Loss $\mathcal{L}_{\text{C}}$}. The contact loss ensures the hand approaches and establishes substantial contact with the object, resulting in a stable grasp. It measures the distance between hand vertices and their closest corresponding object surface vertex:
\begin{equation}
    \mathcal{L}_{\text{C}} = \sum_k \mathcal{L}^2(\mathbf{h}_k, \mathbf{o}_k^{\text{closest}}),
\end{equation} 
where $\mathbf{h}_k \in \pcvec_h$ is the $k$-th hand vertex and $\mathbf{o}_k^{\text{closest}} \in \pcvec_o$ is its closest point on the object mesh.\\

\noindent\textbf{Dynamic Fingertip Loss $\mathcal{L}_{\text{DF}}$}. This loss mimics the human grasping process. It is calculated based on the distance between the thumb tip and the other four fingertips:
\begin{equation}
    \begin{aligned}
            \mathcal{L}_{\text{DF}} &= k \sum_{l} \mathcal{L}^2(\mathbf{x}_{\text{thumb}}, \mathbf{x}_l).
            % k&=\text{OptiStep} - 100.
    \end{aligned}
\end{equation}
$\mathbf{x}_{\text{thumb}}$ is the 3D joint position of the thumb tip and $\mathbf{x}_{l}$ represent 3D joint positions of the other four fingertips. $k$ is the dynamic coefficient, which is negative in the early stages of the optimization (step$<$100) to keep the hand open. In later stages, the coefficient is positive to close the hand towards a stable grasp. \\

\noindent\textbf{Control Loss $\mathcal{L}_{\text{Ctrl}}$}. This loss is designed to ensure that the grasp direction will not deviate from the pre-defined direction during the optimization process. We compute it as the cosine similarity between the wrist vector $\mathbf{v}_{\text{wrist}}$, i.e., the vector pointing from the wrist to the object center, and the grasp direction $\mathbf{v}_{\text{grasp}}$: 
\begin{equation}
    \mathcal{L}_{\text{Ctrl}} = 1 - \frac{\mathbf{v}_{\text{wrist}} \cdot \mathbf{v}_{\text{grasp}}}{|\mathbf{v}_{\text{wrist}}| |\mathbf{v}_{\text{grasp}}|}.
\end{equation}

%\input{sections/figures/fig_6d}


\noindent The learning rate is initially set to 0.003 and decays by 10\% every 100 steps. The entire optimization process takes 500 steps to obtain the final grasping pose. We set the coefficients $\alpha$, $\beta$, $\gamma$, $\delta$ to 1.5, 3, 0.1, and 1, respectively.

\subsection{Handover Motion Generation}
 To generate handover motions, we pass the grasp reference pose $\boldsymbol{\Phi}_{\text{grasp}}$ to our improved variant of D-Grasp \cite{christen:2022:dgrasp} and initialize the hand in the pre-grasp pose $\boldsymbol{\Phi}_{\text{pre}}$. The D-Grasp model takes as input the grasp reference pose and a target 6D object pose. It then generates human motions that approach, grasp, and bring the object into the target pose. In contrast to vanilla D-Grasp, we augment the observation space with information about the object shape to make it more generalizable to unseen objects. Specifically, we compute the signed-distance information \cite{zhang2021manipnet} by sampling the object's signed-distance field for each hand joint, which we add to D-Grasp by concatenating it to the original observation space \cite{christen:2022:dgrasp}.




We generate a training set of grasp reference poses with our optimization on the DexYCB~\cite{chao2021dexycb} object set, which we use as guidance to train D-Grasp. After training the model, we generate grasp reference poses on a larger variety of objects. We synthesize human motions by passing these grasp pose references to the trained D-Grasp model. As our optimization allows control of the approaching direction, we sample grasp directions that are pointing towards the robot. Furthermore, we sample random target object 6D poses within the robot's workspace which serve as handover locations. Lastly, we filter out sequences that fail to grasp the object and reach the target 6D object pose. 




\section{Augmenting Handover Training}
\label{sec:aug_h2r}
To train the robot, we follow the framework in Chapter \ref{ch:handovers:handoversim2real}. Instead of training with trajectories from the DexYCB dataset \cite{chao2021dexycb}, we simulate the human motions in the training environment using our synthetic data. The synthetic human motions are replayed in the simulation during training, following the HandoverSim procedure \cite{chao2022handoversim}. Our method takes as input egocentric RGB-D images. We compute a segmented point cloud (see \figref{fig:synh2r:method_overview}) that is passed through PointNet++ \cite{qi2017pointnet++} to compute a feature that serves as input to our control policy. The control policy is a neural network that predicts actions that are applied to the robot. Given the updated state, the new point cloud is computed and passed to our policy. The training follows a two-stage procedure. In the pre-training stage, we train in a setting where the human has come to a stop before the robot starts moving. This allows us to leverage expert trajectories from motion and grasp planning \cite{wang2020manipulation}. To avoid collisions between the robot and the human, we sample grasps that are opposed to the input direction used in the static grasp generation (cf. \secref{sec:static_grasp_gen}). In the fine-tuning stage, we train the robot in a setting where the human and robot move simultaneously. Since we cannot use open-loop motion and grasp planning in this setting, we utilize a frozen version of the pre-trained policy as expert. Our control policy is trained in actor-critic fashion using a mix of RL-based, behavior cloning, and auxiliary losses as proposed in \cite{wang2021goal}. Please see Chapter \ref{ch:handovers:handoversim2real} for more details about the overall training procedure and the definition of the losses.



==> chapters/05_handover/synh2r/sections/05_experiments.tex <==
\section{Experiments}
\label{sec:synh2r:experiments}

\subsection{Experimental Details}
We generate a train and test set of human handover motions using our method on a subset of ShapeNet objects \cite{chang2015shapenet}. We adjust the size of the objects based on the dimensions specified in ACRONYM~\cite{eppner2020acronym}. To eliminate objects that are too large to grasp for the gripper, we exclude those with a minimal width exceeding 0.15m along the grasp direction.
Our train set comprises 1175 objects and a total of 2230 right-handed handover motions, whereas our test set contains 1174 objects and 4436 handover motions. The test set also includes left-handed motions, which we generate by mirroring the synthesized right-handed motions. As target object 6DoF handover poses, we randomly sample position offsets from the object's initial position within a range of $[-15, 15]$ cm in $x$- and $y$-directions and $[10, 35]$ cm in $z$-direction. For a fair comparison between training on real motion capture and synthetic motions, we use the same training procedure and hyperparameters from \cite{christen:2023:handoversim2real} for both variants. We use a single NVIDIA V100 GPU for training and observe similar convergence times in both data settings.


\input{\dir/synh2r/sections/tables/table_related}
 

\subsection{Baselines}
We experiment with two relevant grasping policies~\cite{christen:2023:handoversim2real,wang2021goal}. GA-DDPG \cite{wang2021goal} is a method for vision-based grasping of rigid objects. Christen \etal~\cite{christen:2023:handoversim2real} is a learning-based method for human-to-robot handovers from point clouds. We use their pre-trained models for evaluation. For \cite{christen:2023:handoversim2real}, we also train on our synthetic data as described in \secref{sec:aug_h2r}. Furthermore, we include the version of GA-DDPG which was trained in the HandoverSim environment following \cite{christen:2023:handoversim2real}. 

\subsection{Metrics} We follow the efficacy metrics in HandoverSim \cite{chao2022handoversim}. We report the overall success rate (\textit{success}). A handover is considered a success if the robot grasps the object and moves it to a goal location without dropping or colliding with the human. We distinguish between the three failure cases of human collision (\textit{contact}), object dropping (\textit{drop}), and timeout if the object is not reached (\textit{timeout}). Since we do not focus on improving the efficiency of handovers in this chapter, we omit the efficiency metrics from HandoverSim from the experiments. 

\subsection{Benchmark Evaluation}
In this experiment, we compare our framework (Christen \etal~\cite{christen:2023:handoversim2real} trained with synthetic data) against baselines on the HandoverSim~\cite{chao2022handoversim} test split (i.e., with real human motions from DexYCB~\cite{chao2021dexycb}). Furthermore, we conduct evaluations on our new synthetic test set to assess generalization to unseen objects and human motions at a larger scale. We report the results in \tabref{tab:synh2r:quantitative} and indicate the dataset each model was trained on. We differ between the \textit{w/ hold} setup, where the robot only starts moving once the human has stopped, and the \textit{w/o hold} setup, where the robot and the human move at the same time. See our supplementary video\footnote{\href{https://eth-ait.github.io/synthetic-handovers}{eth-ait.github.io/synthetic-handovers}} for qualitative examples of our method and the baselines.

\input{\dir/synh2r/sections/tables/table_main}

\noindent\textbf{HandoverSim}
Our method outperforms the GA-DDPG \cite{wang2021goal} baselines, and reaches comparable performance with Christen \etal~\cite{christen:2023:handoversim2real} trained on DexYCB, e.g., a success rate of 70.60\% for our data and 68.75\% for DexYCB data in the \textit{w/o hold} setting. This result is important, as it shows that using purely synthetic human motion data can match the baseline trained on real human motion data. There is a slight drop in performance for synthetic training data compared to DexYCB in the \textit{w/ hold} setting (from 75.23\% to 71.51\%), which we hypothesize is because the HandoverSim test objects are included in the DexYCB train set, whereas our synthetic data does not contain any of the test objects.

\noindent\textbf{Synthetic Test Set}
We compare against baselines on the new synthetic test set that includes 1174 unseen objects (\tabref{tab:synh2r:quantitative} right). Notably, the success rate of the baselines drops when evaluated on a large set of unseen objects. In contrast, training on our synthetic data has significantly higher success rates in both the \textit{w/ hold} and the \textit{w/o hold} setting (e.g., a 20\% relative increase in success rate over the most related baseline \cite{christen:2023:handoversim2real}). This indicates that our synthetic training set improves generalization to unseen objects. The decrease in success rate for all methods on the synthetic test set is expected, as it includes unseen objects and hence a much wider variety of different shapes. While the human-robot collisions (\textit{contact}) remain relatively low on the synthetic test set, the object drop rate increases the most, e.g., in the \textit{w/o hold} setting from 17.82\% on HandoverSim to 32.84\% on the synthetic test set for \cite{christen:2023:handoversim2real} trained on DexYCB. This shows that the methods struggle to find feasible grasps on unseen objects. 

\input{\dir/synh2r/sections/tables/table_ablations}

\subsection{Ablations}
We ablate our synthetic data generation pipeline by comparing it against a variant where we use GraspTTA \cite{jiang2021hand} (\textit{w/ GraspTTA)} instead of our method to generate grasp references for D-Grasp. Furthermore, we analyze the influence of the size of the synthetic train set on the test performance. We report the results on the synthetic test set in \tabref{tab:synh2r:ablation}. We find that a larger training set of synthetic data helps with generalization to unseen objects and human motions, as shown by the decreased performance when only 50\% or 25\% of the synthetic training set are used for training. Our grasp generator can generate more suitable grasps for handovers than GraspTTA, as shown by the relative increase of 10\% in success rate. This implies that the conditioning on the grasping direction is favorable for handover policy training. Note that the ShapeNet objects used are within the training distribution of GraspTTA, as it is trained on Obman \cite{hasson2019learning}, and it is likely to perform worse on unseen objects.


\input{chapters/05_handover/synh2r/sections/figures/user_study_fig}

\subsection{Sim-to-Real Evaluation}
Finally, we transfer the policy trained with our synthetic dataset onto a real robotic platform (system \textit{A}) and compare it with the policy trained on DexYCB from~\cite{christen:2023:handoversim2real} (system \textit{B}), as shown in \figref{fig:synh2r:user}. We seek to answer the question: \textit{Can a person differentiate these two systems from interacting with them?} To answer this, we run a human evaluation with 8 participants. For each participant, the experiment consists of two phases. In the first phase, we let the participant hand over three YCB objects, each to both systems once. After each handover, we inform the participant which system is used (\textit{A} or \textit{B}). In the second phase, we use the 10 household objects selected in~\cite{yang2021reactive} (see Fig.~6 in~\cite{yang2021reactive}) and ask each participant to hand over each object to the robot just once. We randomly sample a system for each object and equally distribute the choices of the two systems (i.e., \textit{A} for 5 objects and \textit{B} for the other 5). In this phase, we do not disclose the chosen system to the participant. After each handover, we ask the participant to make a guess of the chosen system based on the interaction. In the end, we found the two systems both performing competently, exhibiting over 90\% handover success rate (45/50 for \textit{A} and 48/50 for \textit{B}). The classification accuracies from the participants are: (8/10, 6/10, 4/10, 10/10, 10/10, 6/10, 6/10, 10/10) (random guessing is expected to get 5/10). Four of them have an accuracy less or equal to 6/10, struggling to tell apart the two systems. Among the other four, two of them answered ``felt equal'' in a forced choice question between ``preferred \textit{A}'', ``preferred \textit{B}'', and ``felt equal''. They also commented that the systems can be distinguished due to their subtly different tendencies in the approaching direction (the baseline policy tends to have a slight left tilt before handover). This may have resulted from the randomness in training. We provide more qualitative examples in Figures \ref{fig:synh2r:qual_examples} and \ref{fig:synh2r:closeup}. Overall, this result suggests that our system trained purely on synthetic data is performing closely to a system trained on real data.


\input{chapters/05_handover/synh2r/sections/figures/qualitative}

==> chapters/05_handover/synh2r/sections/06_conclusion.tex <==
\section{Conclusion}
In this chapter, we have introduced a framework to generate synthetic human motions for handover training. To generalize to a large scale of unseen objects, our method combines a non-learning based grasp optimizer with an RL-based policy. Our grasp optimization is conditioned on the approaching direction, which allows replicating realistic human handover motions that face towards the robot. We have generated a synthetic train and test set with 100x number of objects compared to the captured dataset. We have then integrated the synthetic human motions into simulation to train a robotic policy with our previously established handover framework (Chapter \ref{ch:handovers:handoversim2real}). In our experiments, we have demonstrated that training with our synthesized motions performs on par compared to training with motion capture data on the HandoverSim benchmark \cite{chao2022handoversim}. On our large scale synthetic test set, we have shown performance improvements when training with our synthetic data, indicating better generalization to unseen objects. In our user study, we have observed that users find it difficult to distinguish a model trained on real captured data from a model trained with synthetic data. This has an important implication for future human-robot interaction tasks, particularly in situations where the collection of human data is expensive, making synthetic data a viable alternative.



==> chapters/05_handover/synh2r/sections/figures/fig_gripper.tex <==
\begin{figure}[t]
\begin{center}
   \includegraphics[width=1.0\textwidth]{\dir/synh2r/sections/figures/gripper_v2.pdf}
\end{center}
   \vspace{-0.35cm}
   \caption{\textbf{Grasp Reference Generation.} Given a grasp direction $\mathbf{v}_{\text{grasp}}$ and an object mesh $\pcvec_o$, our method generates a pre-grasp pose $\boldsymbol{\Phi}_{\text{pre}}$ and grasp reference pose $\boldsymbol{\Phi}_{\text{grasp}}$.}
\label{fig:synh2r:gripper}
\end{figure}

==> chapters/05_handover/synh2r/sections/figures/fig_method.tex <==
\begin{figure*}[t]
\begin{center}
   \includegraphics[width=\textwidth]{\dir/synh2r/sections/figures/pipeline.pdf}
\end{center}
    \vspace{-4mm}
   \caption{\textbf{Method Overview.} Our framework contains a handover motion generation stage and a H2R handover training stage.}

\label{fig:synh2r:method_overview}
\end{figure*}




==> chapters/05_handover/synh2r/sections/figures/fig_teaser.tex <==
\begin{figure}
\begin{center}
   \includegraphics[width=1.0\textwidth]{\dir/synh2r/sections/figures/teaser.pdf}
\end{center}
   \vspace{-0.25cm}
   \caption{\textbf{Overview of our framework.} We train a robot to perform human-to-robot handovers using synthetic human motions. We transfer to a real robot and evaluate on a large synthetic test set of unseen objects and human motions.}

\label{fig:synh2r:teaser}
\end{figure}

==> chapters/05_handover/synh2r/sections/figures/qualitative.tex <==
\begin{figure}[ht]
    \centering

    % \begin{minipage}
    % First row of images
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{\dir/synh2r/sections/figures/seqs/mug_1.jpg}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{\dir/synh2r/sections/figures/seqs/mug_2.jpg}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{\dir/synh2r/sections/figures/seqs/mug_3.jpg}
    \end{subfigure}
    \parbox{\textwidth}{\centering \small{Mug} \par}
    \vspace{0.2em} % Space between the row and the pseudo-caption

    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{\dir/synh2r/sections/figures/seqs/newspaper_1.jpg}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{\dir/synh2r/sections/figures/seqs/newspaper_3.jpg}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{\dir/synh2r/sections/figures/seqs/newspaper_2.jpg}
    \end{subfigure}
    \parbox{\textwidth}{\centering \small{Newspaper} \par}
    \vspace{0.2em}
    
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{\dir/synh2r/sections/figures/seqs/towel_1.jpg}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{\dir/synh2r/sections/figures/seqs/towel_2.jpg}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{\dir/synh2r/sections/figures/seqs/towel_3.jpg}
    \end{subfigure}
    \parbox{\textwidth}{\centering \small{Towel} \par}
    \vspace{0.2em}

    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{\dir/synh2r/sections/figures/seqs/remote_1.jpg}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{\dir/synh2r/sections/figures/seqs/remote_2.jpg}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{\dir/synh2r/sections/figures/seqs/remote_3.jpg}
    \end{subfigure}
    \parbox{\textwidth}{\centering \small{Remote} \par}

    \vspace{-2mm} 
    \caption{\textbf{Qualitative examples.} Users interacting with our model trained on synthetic human motions.}
    \label{fig:synh2r:qual_examples}
\end{figure}

\begin{figure}[ht]
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{\dir/synh2r/sections/figures/seqs/banana_close.png}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{\dir/synh2r/sections/figures/seqs/plate_close.jpg}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{\dir/synh2r/sections/figures/seqs/box_close.png}
    \end{subfigure}
    \caption{\textbf{Close up examples.} Zoomed in images of handovers.}
    \label{fig:synh2r:closeup}
\end{figure}

==> chapters/05_handover/synh2r/sections/figures/user_study_fig.tex <==
\begin{figure}[t]
    \centering

    % \begin{minipage}
    % First row of images
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{\dir/synh2r/sections/figures/seqs/synh2r_1.jpg}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{\dir/synh2r/sections/figures/seqs/synh2r_2.jpg}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{\dir/synh2r/sections/figures/seqs/synh2r_3.jpg}
    \end{subfigure}
    \parbox{\textwidth}{\centering \small{User interacting with SynH2R.} \par}
    \vspace{0.5em} % Space between the row and the pseudo-caption

    
    
    
    % Second row of images
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{\dir/synh2r/sections/figures/seqs/handoversim2real_1.jpg}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{\dir/synh2r/sections/figures/seqs/handoversim2real_2.jpg}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{\dir/synh2r/sections/figures/seqs/handoversim2real_3.jpg}
    \end{subfigure}
    \parbox{\textwidth}{\centering \small{User interacting with our previous system (Chapter \ref{ch:handovers:handoversim2real}).} \par}
    % Caption for the second set of images
    \vspace{-2mm} 
    \caption{In our real world evaluations, we let users interact with a variant trained with real human motion data and a variant trained with our synthetic human motion data. After an initial training phase with both models, users had to indicate which model they believe they are interacting with}
    \label{fig:synh2r:user}
\end{figure}

==> chapters/05_handover/synh2r/sections/tables/table_ablations.tex <==
\begin{table}[t!]
 \vspace{-0mm}
 \centering
 \small
 % \setlength{\tabcolsep}{6pt}
  \caption{\textbf{Ablation of our framework.} We compare our method against a variant trained with grasp references generated using GraspTTA \cite{jiang2021hand} and different amount of data from our synthetic train set (25\% and 50\%). The best result is marked in bold, the second best result is underlined.}
   \vspace{-1mm}
  \resizebox{0.85\columnwidth}{!}{%
 \begin{tabular}{l|cccc}

  \hline
  \multirow{2}{*}{Synthetic Test Set} & \multirow{2}{*}{success (\%)} &  \multicolumn{3}{c}{failure (\%)} \\
  & & contact & drop & timeout \\
  \midrule

   w/ GraspTTA \cite{jiang2021hand} & \underline{50.33} & ~\textbf{6.12} & 31.89  &  \underline{11.64}        \\
   \gc Ours - 25\% & \gc 47.23  & \gc ~8.08 & \gc \textbf{25.75} & \gc 18.93         \\

   Ours - 50\%  & 49.21  & 10.75 & 27.22 & 12.80          \\

  \gc Ours & \gc \textbf{55.94} & \gc ~\underline{7.53} & \gc \underline{25.89} & \textbf{10.63} \gc \\ 
%   Ours (hand avg + pred)  w/o hold & 43.73 & tbd & tbd & tbd  & 16.3 & ~21.5 & ~18.40 \\ 
  \hline
 \end{tabular}
 }

 \label{tab:synh2r:ablation}
\end{table}

==> chapters/05_handover/synh2r/sections/tables/table_main.tex <==
\begin{table*}[t]
 % \vspace{-2mm}
 \centering
 \small

 \caption{\textbf{Benchmark Evaluation.} We conduct experiments on HandoverSim and on the Synthetic Test Set.}

\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{l|l|l|cccc|cccc}

  \hline
  & & & \multicolumn{4}{c|}{HandoverSim Test Set (DexYCB)} & \multicolumn{4}{c}{Our Synthetic Test Set} \\ \midrule
  & \multirow{2}{*}{Method} & \multirow{2}{*}{Training Data} & \multirow{2}{*}{success (\%)} & \multicolumn{3}{c|}{failure (\%)} & \multirow{2}{*}{success (\%)} & \multicolumn{3}{c}{failure (\%)} \\
  & & & & contact & drop & timeout & & contact & drop & timeout \\
  \hline
  \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{w/ hold}}}
  & GA-DDPG~\cite{wang2021goal} & ShapeNet~\cite{chang2015shapenet} & 50.00         & ~\textbf{4.86} &  19.44        &  25.69 &   31.22   &  16.39      &   43.85    &   ~\textbf{8.54}    \\
  & \gc GA-DDPG finetuned~\cite{christen:2023:handoversim2real} & \gc DexYCB~\cite{chao2021dexycb} & \gc 57.18        & \gc ~6.48 &  \gc 27.08          &  \gc ~9.26 &   \gc 40.67  &  \gc  15.70    &  \gc 36.24   &   \gc  ~7.38  \\ 
  & Christen et. al~\cite{christen:2023:handoversim2real}  & DexYCB~\cite{chao2021dexycb} &  \textbf{75.23} & ~9.26 & \textbf{13.43} &  ~\textbf{2.08} & 46.57   & 13.90 &  28.68  &  10.85   \\
  & \gc Christen et. al~\cite{christen:2023:handoversim2real} & \gc Our Synthetic & \gc 71.51  & \gc ~7.87 & \gc 15.30 & \gc ~5.32  & \gc \textbf{56.25} & \gc ~\textbf{8.06} & \gc \textbf{23.50} & \gc 12.17 \\
%   & \gc Ours + grasp pred. & \gc 71.07 & \gc 5.43 & \gc tbd & \gc tbd  & \gc ~6.00 & \gc 16.20 & \gc ~6.73 \\ 
%   Ours (hand avg + pred)  w/o hold & 43.73 & tbd & tbd & tbd  & 16.3 & ~21.5 & ~18.40 \\ 
% 67.84	9.95	15.52	6.726666667 0.7151	0.0787	0.1530	0.0532 
\hline

  \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{w/o hold}}}
  
  & GA-DDPG~\cite{wang2021goal} & ShapeNet~\cite{chang2015shapenet} &  36.81         &  ~9.03          &  25.00          &  29.17  & 23.90 & 18.26  & 48.67   &  ~9.17 \\
  & \gc GA-DDPG finetuned~\cite{christen:2023:handoversim2real} & \gc DexYCB~\cite{chao2021dexycb} & \gc 54.86         & \gc ~\textbf{6.71} &  \gc 26.39          & \gc 12.04 & \gc 37.53 & \gc 12.32      & \gc 35.03  & \gc  16.44  \\
  &  Christen et. al~\cite{christen:2023:handoversim2real} & DexYCB~\cite{chao2021dexycb} &   68.75  & ~8.80 &  17.82 &   ~\textbf{4.63} & 43.20 & 10.92 & 32.84   & 13.02 \\ 
 
  & \gc Christen et. al~\cite{christen:2023:handoversim2real} & \gc Our Synthetic & \gc \textbf{70.60} & \gc ~7.18 & \gc \textbf{16.67} & \gc ~5.56  & \gc \textbf{55.94} & \gc ~\textbf{7.53} & \gc \textbf{25.89} & \gc \textbf{10.63} \\  
%   & \gc Ours + grasp pred & \gc 70.37 & \gc 4.860 & \gc tbd & \gc tbd  & \gc 7.64 & \gc ~14.71 & \gc ~6.95 \\  0.2390	0.1826	0.4867	0.0917 
\bottomrule
  
\end{tabular}
}


 \label{tab:synh2r:quantitative}
\end{table*}

==> chapters/05_handover/synh2r/sections/tables/table_main_real.tex <==
\begin{table}[t]
 % \vspace{-2mm}
 \centering
 \small
 % \setlength{\tabcolsep}{6pt}
\caption{\textbf{HandoverSim Benchmark Evaluation DexYCB.}}
\begin{tabular}{l|l|cccc}
  \hline
  & DexYCB & \multirow{2}{*}{success (\%)} & \multicolumn{3}{c}{failure (\%)} \\
  & & & contact & drop & timeout \\
  \hline
  \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Static}}}
  & GA-DDPG [5]   & 50.00         & ~\textbf{4.86} &  19.44          &  25.69      \\
  & \gc Christen et. al    &  \gc \textbf{75.23} & \gc ~9.26 & \gc \textbf{13.43} & \gc ~\textbf{2.08}   \\
  & Ours  & 67.84 & 9.95 & 15.52       &  6.73 \\
%   & \gc Ours + grasp pred. & \gc 71.07 & \gc 5.43 & \gc tbd & \gc tbd  & \gc ~6.00 & \gc 16.20 & \gc ~6.73 \\ 
%   Ours (hand avg + pred)  w/o hold & 43.73 & tbd & tbd & tbd  & 16.3 & ~21.5 & ~18.40 \\ 
% 67.84	9.95	15.52	6.726666667
\hline

  \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Dyn.}}}
  
  & GA-DDPG   &  36.81         &  ~9.03          &  25.00          &  29.17       \\
  & \gc Christen et. al  & \gc  68.75  & \gc ~8.80 &  \gc 17.82 &  \gc  ~\textbf{4.63}  \\
 
  & Ours & \textbf{69.90} & \textbf{5.80} & \textbf{16.45} & 7.88   \\
%   & \gc Ours + grasp pred & \gc 70.37 & \gc 4.860 & \gc tbd & \gc tbd  & \gc 7.64 & \gc ~14.71 & \gc ~6.95 \\ 
  
\bottomrule
  
 \end{tabular}



 \label{tab:synh2r:quantitative}
\end{table}

==> chapters/05_handover/synh2r/sections/tables/table_main_syn.tex <==
\begin{table}[t]
 % \vspace{-2mm}
 \centering
 \small
 % \setlength{\tabcolsep}{6pt}
 
 \caption{\textbf{HandoverSim Benchmark Evaluation Synthetic.}}
 \begin{tabular}{l|l|cccc}

  \hline
  & Synthetic & \multirow{2}{*}{success (\%)} & \multicolumn{3}{c}{failure (\%)} \\
  & & & contact & drop & to \\
  \hline
  \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Static}}}
  & GA-DDPG \cite{wang:corl2021b} &   34.54   &  11.50      &   45.31    &   \textbf{8.66}      \\
  & \gc Christen \etal~\cite{christen2023handoversim2real}  & \gc 49.64   & \gc 11.85 &  \gc  27.43  &  \gc 11.08   \\
  & Ours & \textbf{61.68} & \textbf{8.20} & \textbf{20.54} & 9.78   \\
%   & \gc Ours + grasp pred. & \gc 71.07 & \gc 5.43 & \gc tbd & \gc tbd  & \gc ~6.00 & \gc 16.20 & \gc ~6.73 \\ 
%   Ours (hand avg + pred)  w/o hold & 43.73 & tbd & tbd & tbd  & 16.3 & ~21.5 & ~18.40 \\ 

\hline

  \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Dyn.}}}
  
  & GA-DDPG \cite{wang:corl2021b} &  6.67 & 12.76 &  55.55  & 25.02 \\
  % & GA-DDPG ft &  6.67 & 12.76 &  55.55  & 25.02 \\
  & \gc Christen \etal~\cite{christen2023handoversim2real}  & \gc 34.04 & \gc 14.49 & \gc 35.03           & \gc 16.44      \\
 
  & Ours   & \textbf{53.16} & \textbf{7.17} & \textbf{29.46} & \textbf{10.22}    \\
%   & \gc Ours + grasp pred & \gc 70.37 & \gc 4.860 & \gc tbd & \gc tbd  & \gc 7.64 & \gc ~14.71 & \gc ~6.95 \\ 
\bottomrule
  
 \end{tabular}

 \label{tab:synh2r:quantitative}
\end{table}

==> chapters/05_handover/synh2r/sections/tables/table_related.tex <==
\begin{table}
\centering
\begin{center}
\caption{\textbf{Evaluation Sets Overview.} Comparison between the number of objects and test configurations used in the most related works and ours.}
\vspace{-0.1cm}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{l|cc}
   \toprule
    Benchmark & Num Objects & Test Configurations \\
    \midrule
    Sanchez-Matilla \etal~\cite{sanchezmatilla2020benchmark} & ~~~4 & ~288 \\ 
    Rosenberger \etal~\cite{rosenberger2021object} & ~~13  & ~520 \\
    Yang \etal~\cite{yang2021reactive}    &  ~~26  & ~156 \\
    HandoverSim ('S0') \cite{chao2022handoversim}    &  ~~18 & ~144 \\
    \textbf{Ours} &  \textbf{1174} & \textbf{4436} \\
   \bottomrule
   
\end{tabular}
}
\label{tab:synh2r:related}
\end{center}


\end{table}

==> frontbackmatter/cv.tex <==
%*******************************************************
% CV
%*******************************************************
\pdfbookmark[1]{Curriculum Vitae}{cv}

\bigskip

\begingroup
\let\clearpage\relax
\let\cleardoublepage\relax
\let\cleardoublepage\relax
\chapter*{Curriculum Vitae}

\section*{Personal data}

\noindent\cvleft{Name}%
\cvright{Sammy Joe Christen}\\
%
\cvleft{Date of Birth}%
\cvright{July 26, 1991}\\
%
\cvleft{Place of Birth}%
\cvright{Lucerne, Switzerland}\\
%
\cvleft{Citizen of}%
\cvright{Switzerland}

\section*{Education}

\noindent\cvleft{2016 --~2018}%
\cvright{%
  ETH Zurich \\
  Zurich, Switzerland\\
  \emph{Final degree:} Master of Science
}\vspace{0.75em}


\noindent\cvleft{2012 --~2015}%
\cvright{%
  ETH Zurich \\
  Zurich, Switzerland\\
  \emph{Final degree:} Bachelor of Science
}\vspace{0.75em}

\noindent\cvleft{2004-~2011}%
\cvright{%
  Kantonsschule Beromünster (High School)\\
  Beromünster, Switzerland
}

\endgroup
